Near-Optimal Algorithms for Private Online Optimization in the Realizable Regime

We consider online learning problems in the realizable setting, where there is a zero-loss solution, and propose new Differentially Private (DP) algorithms that obtain near-optimal regret bounds. For the problem of online prediction from experts, we design new algorithms that obtain near-optimal regret ${O} \big( \varepsilon^{-1} \log^{1.5}{d} \big)$ where $d$ is the number of experts. This significantly improves over the best existing regret bounds for the DP non-realizable setting which are ${O} \big( \varepsilon^{-1} \min\big\{d, T^{1/3}\log d\big\} \big)$. We also develop an adaptive algorithm for the small-loss setting with regret $O(L^\star\log d + \varepsilon^{-1} \log^{1.5}{d})$ where $L^\star$ is the total loss of the best expert. Additionally, we consider DP online convex optimization in the realizable setting and propose an algorithm with near-optimal regret $O \big(\varepsilon^{-1} d^{1.5} \big)$, as well as an algorithm for the smooth case with regret $O \big( \varepsilon^{-2/3} (dT)^{1/3} \big)$, both significantly improving over existing bounds in the non-realizable regime.

==> introduction.tex <==

\section{Introduction}
\label{sec:intro}
% %most papers study DP-SCO -> but modern ML and FL motivate DP-OCO -> not well studied (many gaps) -> we study DP-OCO

We study the problem of differentially private online prediction from experts (DP-OPE), where the algorithm interacts with an adversary for $T$ rounds. In each round, the algorithm picks an expert $x_t \in [d]$ and the adversary chooses a loss function $\ell_t: [d] \to [0,1]$. The algorithm incurs loss $\ell_t(x_t)$ at round $t$, and the goal is to design algorithms that minimize the regret, that is, the cumulative loss compared to the best fixed expert in hindsight, defined as
\begin{equation*}
    Reg_T = \sum_{t=1}^T \ell_t(x_t) -  \min_{x^\star \in [d]} \sum_{t=1}^T \ell_t(x^\star).
\end{equation*}

Online prediction from experts is an important problem in machine learning with numerous applications~\citep{AroraHaKa12}.
Without any privacy restrictions, the power of the adversary (oblivious adversary that picks the losses in advance versus adaptive adversary that picks the losses online in response to the algorithm) does not change the optimal rates for this problem~\citep{cesa2006prediction}. This has perhaps led prior work in private online experts to focus on the strongest notion of adaptive adversaries~\citep{JainKoTh12,SmithTh13,JainTh14,AgarwalSi17}. In this work, we study the problem of DP-OPE against oblivious adversaries as well and show that, somewhat surprisingly, the power of the adversary can significantly affect the optimal rates for this problem.

We consider three types of adversaries: the strongest, \emph{adaptive adversary}, can choose the loss sequence $(\ell_t)_{t=1}^T$ adversarially in an online manner, where the loss $\ell_t$ may depend arbitrarily on the choices made by the algorithm in previous time steps $(x_\ell)_{\ell=1}^{t-1}$. A slightly weaker notion is that of an \emph{oblivious adversary}, which chooses a sequence of loss functions in advance. The weakest adversary is the \emph{stochastic adversary} which chooses a distribution over loss functions and at each round samples a loss function i.i.d.~from this distribution.

In the classical non-private setting, all of these adversarial models are equivalent, in the sense that they all induce an optimal rate of order $\sqrt{T \log d}$~\citep{cesa2006prediction}. We study algorithms that are required to be differentially private, where we view the sequence of loss functions as the dataset and adjacent datasets differ in a single loss function. We note that all our algorithms are private with respect to adaptive adversaries (see~\cref{sec:pre} for precise definitions) and only the utility bounds assume a weaker adversary. 

Under the constraint of \ed-differential privacy, the best existing results obtain regret of order
$$
\sqrt{T \log d} + \min\left( \frac{1}{\diffp} \sqrt{T \log(1/\delta) \log d}, \frac{1}{\diffp} \sqrt{d \log(1/\delta)} \log d \log^2 T \right) 
$$ 
for adaptive adversaries~\citep{JainTh14,AgarwalSi17}. For pure $\diffp$-differential privacy, the best existing regret~\citep{JainTh14} is of order 
$$\sqrt{T \log d} +  \frac{d  \log d \log^2 T}{\diffp}.$$ 
However, none of existing results prove any lower bounds (besides the trivial non-private lower bound $\sqrt{T \log d}$) to certify the optimality of these rates; thus, it is currently unclear whether these rates are optimal for adaptive adversaries, let alone for oblivious and stochastic adversaries.


%\citet{JainKoTh12} first studied DP-OPE and several subsequent papers developed new algorithms with improved rates~\cite{SmithTh13,JainTh14,AgarwalSi17}. However, existing rates for DP-OPE demonstrate a non-negligible privacy cost; yet none of the existing results prove any lower bounds (besides the trivial non-private lower bound) to certify the optimality of these rates. In this paper we develop new algorithms and lower bounds that close some of these gaps.

%This is one of the most fundamental problems in machine learning\hac{add some motivation here}.  DP-OPE has been extensively studied in the last decade~\cite{DworkNaPiRo10,JainKoTh12,SmithTh13,JainTh14,AgarwalSi17}. However, there remain major limitations in our understanding of this problem in the private setting. 




\subsection{Our contributions}
We study DP-OPE for different types of adversaries and develop new algorithms and lower bounds. More precisely, we obtain the following results.

\paragraph{Faster rates for oblivious adversaries (\cref{sec:ub-obl-sd}):} 
We develop new algorithms for DP-OPE with oblivious adversaries based on a lazy version of the multiplicative weights algorithm. For pure $\diffp$-DP, our algorithms obtain regret $$\frac{\sqrt{T} \log d}{\diffp}.$$ 
This is the first algorithm to achieve sub-linear regret for pure DP in the high-dimensional regime $d \ge T$. For approximate \ed-DP, our algorithm achieves regret $$ \sqrt{T \log d } + \frac{T^{1/3} \log^{1/3}(1/\delta) \log d}{\diffp}.$$ 
This essentially demonstrates that the privacy cost for DP-OPE is negligible as long as $\diffp \gg T^{-1/6}$. In contrast, previous work has established privacy cost $\diffp^{-1} \sqrt{T \log d\log(1/\delta)}$ which is larger than the non-private cost even when $\diffp$ is constant and $\delta=1/T$. See~\cref{fig:table-appr,fig:table-pure} for more details.

\paragraph{Separation between adaptive and oblivious adversaries (\cref{sec:lower-bounds}):} 
We prove the first lower bounds for DP-OPE with adaptive adversaries that are stronger than the non-private lower bounds. These bounds show that any private algorithm must suffer linear regret if $\diffp \le 1/\sqrt{T}$ for approximate DP and $\diffp \le 1/10$ for pure DP. As our algorithms for oblivious adversaries obtain sub-linear regret in this regime of privacy parameters, this demonstrates that the oblivious model is significantly weaker than the adaptive model in the private setting (see~\cref{fig:comp}). Moreover, these lower bounds show a separation between pure and approximate DP for DP-OPE with adaptive adversaries as the latter is necessary to obtain sub-linear regret.

\paragraph{Near-optimal rates for stochastic adversaries (\cref{sec:ub-stoch}):}  
We design a general reduction that transforms any algorithm for private stochastic optimization in the offline setting into an algorithm for private online optimization with nearly the same rates (up to logarithmic factors). By building on algorithms for the offline setting~\citep{AsiFeKoTa21}, we obtain regret $O(\sqrt{T\log d} +  \diffp^{-1}\log d \log T)$ for DP-OPE with stochastic adversaries. Moreover, using this reduction with general algorithms for differentially private stochastic convex optimization (DP-SCO)~\citep{FeldmanKoTa20}, we obtain near-optimal regret $O( \sqrt{T} + \diffp^{-1} \sqrt{d} \log T )$ for the problem of DP-OCO (online convex optimization) with stochastic adversaries, improving over the best existing result $\sqrt{T}d^{1/4}/\diffp $~\citep{KairouzMcSoShThXu21}.


%\paragraph{Optimal rates for oblivious adversaries in the realizable setting} (\cref{sec:upper-bounds-realizable}) we also study the realizable setting where the best expert achieves zeros loss, that is,  $L\opt \defeq \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) = 0$. We design new algorithms---one based on sparse-vector and one based on the binary tree mechanism---that obtain near-optimal regret $O(\diffp^{-1} \mathsf{poly}(\log d))$. For $L\opt>0$, we extend these algorithms to achieve regret $O(L\opt \log(T) + \diffp^{-1} \mathsf{poly} (\log d))$, which can offer significant improvements for $L\opt \ll \sqrt{T}$.

\paragraph{Improved rates for DP-OCO (\cref{sec:oco-imp}):}
Building on our improvements for DP-OPE, we improve the existing rates for DP-OCO where the algorithms picks $x_t \in \mc{X} = \{ x \in \R^d: \ltwo{x} \le 1\}$ and the adversary picks $\ell_t : \mc{X} \to \R$. Our rates improve over the rates of~\cite{KairouzMcSoShThXu21} in certain regimes.  


% Distinguishing between adaptive and oblivious adversary.
% New algorithms for DP-OPE and new lower bounds.

% \begin{enumerate}
%     \item Reduction from DP-SCO to DP-OCO against stochastic adversaries.
    
%     \item New algorithms for DP-OPE that improve the rates against oblivious adversaries. First \ed-DP rates that have negligible privacy cost. First $\diffp$-DP rates that are sub-linear. 
    
%     \item Lower bounds for adaptive adversaries. First non-trivial lower bounds that show the cost of privacy in this setting. Separation between adaptive and oblivious adversaries. Separation between pure and approximate DP.
    
%     \item New algorithms for the realizable setting. Near optimal rates $O(\log(d)/\diffp)$.
    
% \end{enumerate}


\renewcommand{\arraystretch}{2}

\begin{table}[h]
\begin{center}
    \begin{subtable}[h]{0.8\textwidth}
		\begin{tabular}{| c | c | c |}
		    \hline
			  & \textbf{\darkblue{Prior work}} & \textbf{\darkblue{This work}}\\
			\hline
			{{\textbf{Stochastic}}} & \multirow{3}{*}{{$ \sqrt{T \log d} + \min\left( \frac{\sqrt{T  \log d}}{\diffp}, \frac{\sqrt{d } \log  d}{\diffp}    \right)$}  } & $   \sqrt{T\log d} +  \frac{\log d }{\diffp} $      \\
			\cline{1-1} \cline{3-3}
			\textbf{{Oblivious}} & & $\sqrt{T \log d } + \frac{T^{1/3}  \log d}{\diffp}$ \\ %& $\Omega \left( \frac{d^2 }{n^2 \diffp^2}   \right)$ \\
			\cline{1-1} \cline{3-3}
			{\textbf{Adaptive}} & & None \\ %& $\Omega \left( \frac{d^2 }{n^2 \diffp^2}   \right)$ \\
			\hline
		\end{tabular}
    \caption{Approximate \ed-DP.}
    \label{fig:table-appr}
\end{subtable}

\vspace{.5cm}
\begin{subtable}[h]{0.8\textwidth}
        \hspace{2cm}
		\begin{tabular}{| c | c | c |}
		    \hline
			  & \textbf{\darkblue{Prior work}} & \textbf{\darkblue{This work}}\\
			\hline
			{\textbf{Stochastic}} & \multirow{3}{*}{{$ \sqrt{T \log d} +  \frac{d \log d}{\diffp}$}  } & $   \sqrt{T\log d} +  \frac{\log d }{\diffp} $      \\
			\cline{1-1} \cline{3-3}
			{\textbf{Oblivious}} & & $\frac{\sqrt{T} \log d}{\diffp}$ \\ %& $\Omega \left( \frac{d^2 }{n^2 \diffp^2}   \right)$ \\
			\cline{1-1} \cline{3-3}
			{\textbf{Adaptive}} & & None \\ %& $\Omega \left( \frac{d^2 }{n^2 \diffp^2}   \right)$ \\
			\hline
		\end{tabular}
    \caption{Pure $\diffp$-DP.}
    \label{fig:table-pure}
\end{subtable}
     \caption{Upper bounds for DP-OPE with different types of adversaries. For readability, we omit logarithmic factors that depend on $T$ and $1/\delta$.}
     \label{tab:temps}
     \end{center}
\end{table}



\begin{figure}[htb] 
  \begin{subfigure}{0.5\textwidth}
    \centering
    \begin{tikzpicture}
%\begin{axis}[
%    axis lines = left,
%    xlabel = \(x\),
%    ylabel = {\(f(x)\)},
%]
\begin{axis}[
width=7.0cm,               %% here, adjust as suitable
%axis y line=center,
%axis x line=left,
%axis lines = middle,  %% instead of above two lines this one is enough
%scaled ticks=false,
%axis equal,
grid=major,
xmax=1,xmin=0,
ymin=0.4,ymax=1.1,
xlabel={$\alpha$},ylabel={$\beta$},
legend style={at={(0.7,0.46)},anchor=north},
tick label style={font=\small}
%legend pos=south east,
]
%Below the red parabola is defined


\addplot+[color=red,domain=0:1,thick,mark=none] {min(max(1/3 + x,1/2),1)};
\addlegendentry{\tiny DP-SD (Cor.~\ref{cor:sd-appr})}

\addplot+[color=blue,domain=1/3:1,thick,mark=none] {min(2/5 + 4*x/5,1)};
\addlegendentry{\tiny Batch DP-SD (Cor.~\ref{cor:sd-batch})}

\addplot+[color=black,domain=0:1,thick,mark=none] {min(max(1/2 + x,1/2),1)};
\addlegendentry{\tiny Prior work}

\addplot+[color=black,domain=0:1/2,thick,dashed,mark=none] {max(1/2,2*x)};
\addlegendentry{\tiny LB (adaptive adversary)}

% \addplot+[color=black,domain=0:1,thick,dashed, mark=none] {min(max(1/3 + 2*x/3,1/2),1)};
% \addlegendentry{Conjecture}

%Here the blue parabola is defined

\end{axis}
\end{tikzpicture}
    \caption{Approximate \ed-DP}
  \end{subfigure}%
  \begin{subfigure}{0.5\textwidth}
    \centering
    \begin{tikzpicture}
%\begin{axis}[
%    axis lines = left,
%    xlabel = \(x\),
%    ylabel = {\(f(x)\)},
%]
\begin{axis}[
width=7.0cm,               %% here, adjust as suitable
%axis y line=center,
%axis x line=left,
%axis lines = middle,  %% instead of above two lines this one is enough
%scaled ticks=false,
%axis equal,
grid=major,
xmax=1,xmin=0,
ymin=0.4,ymax=1.1,
xlabel={$\alpha$},%ylabel=\Large{$\beta$},
legend style={at={(0.7,0.4)},anchor=north},
tick label style={font=\small}
%legend pos=south east,
]
%Below the red parabola is defined


\addplot+[color=red,domain=0:1,thick,mark=none] {min(max(1/2 + x,1/2),1)};
\addlegendentry{\tiny DP-SD (Cor.~\ref{cor:sd-appr})}

% \addplot+[color=blue,domain=1/3:1,thick,mark=none] {min(2/5 + 4*x/5,1)};
% \addlegendentry{DP-SD with batch (Cor.~\ref{cor:sd-batch})}

\addplot+[color=black,domain=0:1,thick,mark=none] {1};
\addlegendentry{\tiny Prior work}

\addplot+[color=black,domain=0:1/2,thick,dashed,mark=none] {1};
\addlegendentry{\tiny LB (adaptive adversary)}

% \addplot+[color=black,domain=0:1,thick,dashed, mark=none] {min(max(1/3 + 2*x/3,1/2),1)};
% \addlegendentry{Conjecture}

%Here the blue parabola is defined

\end{axis}
\end{tikzpicture}
    \caption{Pure $\diffp$-DP}
  \end{subfigure}
  \caption{Regret bounds for private prediction from experts against oblivious adversaries for the high-dimensional regime $d \ge T$. 
We denote the privacy parameter $\diffp = T^{-\alpha}$ and regret $T^\beta$, and plot $\beta$ as a function of $\alpha$ (ignoring logarithmic factors).  }\label{fig:comp}
\end{figure}







\subsection{Related work}
\citet{DworkNaPiRo10} were the first to study differentially private learning in the online setting and introduced the binary tree mechanism which is an important building block of many private algorithms in the online setting. In our context of online prediction from experts, there has been several works that study this problem under the constraint of differential privacy~\citep{JainKoTh12,SmithTh13,JainTh14,AgarwalSi17}. The best existing algorithms depend on the dimensionality regime: in the high-dimensional setting, \citet{JainTh14} developed an algorithm based on follow-the-regularized-leader (FTRL) with entropy regularization that achieves regret $O(\diffp^{-1}\sqrt{T \log d \log(1/\delta)})$ for \ed-DP. For low dimensional problems, \citet{AgarwalSi17} developed an improved algorithm that uses the binary tree mechanism to estimate the running sum of the gradients in the FTRL framework. Their algorithm achieves regret $O(\sqrt{T\log d} + \diffp^{-1} d \log d \log^2 T)$  for $\diffp$-DP. Moreover, extending their algorithm to \ed-DP results in regret  $O(\sqrt{T\log d} + \diffp^{-1} \sqrt{d \log(1/\delta)} \log d \log^2 T)$.

A slightly related and somewhat easier problem is that of differentially private stochastic convex optimization (DP-SCO) which has been extensively investigated recently~\citep{BassilySmTh14,BassilyFeTaTh19,FeldmanKoTa20,AsiFeKoTa21,AsiDuFaJaTa21}. In DP-SCO, we are given $n$ samples from some distribution and we wish to minimize the excess population loss. In contrast to the online setting, here all $n$ samples are given to the algorithm and it is required to produce only one model; this makes the online version harder as the algorithm has to output a model at each time-step. However, we note that our reduction in~\cref{sec:ub-stoch} shows that DP-SCO is essentially as hard as DP-OCO with stochastic adversaries (up to logarithmic factors). For oblivious and adaptive adversaries, the online setting may be harder as it allows general loss functions that are not necessarily generated from a distribution.

Perhaps most closely related to our problem in the non-private setting is online learning with limited switching~\citep{KalaiVe05,GeulenVoWi10,AltschulerTa18,chen2020minimax,ShermanKo21}. In this setting, the algorithm aims to minimize the regret when having a budget of at most $S$ switches, that is, it can update its decision at most $S$ times. This constraint is (informally) somewhat related to privacy as the less you update the model, the less information is leaked about the data. The ideas developed in this literature turn out to be useful for our DP-OPE setting. Indeed, our algorithms in~\cref{sec:ub-obl-sd} build on ideas from~\cite{GeulenVoWi10} which developed a lazy version of multiplicative weights to limit the number of switches. Moreover,
similarly to our results, the hardness of online learning problems with limited switching can depend on the power of the adversary. For example, for OCO with limited switching, the optimal rate is $\sqrt{T} + T/S$ for oblivious adversaries and $\sqrt{T} + T/\sqrt{S}$ for adaptive adversaries~\citep{chen2020minimax,ShermanKo21}. Despite of these similarities, our results do not establish a fundamental connection between privacy and switching constraints and we leave this as an open question for future research.


% Talk about: 

% 1. non-private OPE and OCO~\cite{KalaiVe05,Hazan16,GeulenVoWi10}

% 2. limited switching OCO~\cite{GeulenVoWi10,AltschulerTa18,ShermanKo21}

% 2. DP online (general)~\cite{DworkNaPiRo10}

% 3. DP-OPE~\cite{JainKoTh12,SmithTh13,JainTh14,AgarwalSi17}  + a little DP-OCO~\cite{KairouzMcSoShThXu21}

% 4. DP-SCO (a little)~\cite{BassilyFeTaTh19,FeldmanKoTa20,AsiFeKoTa21,AsiDuFaJaTa21}

% \begin{enumerate}
%     \item \cite{DworkNaPiRo10} first paper on online DP
%     \item \cite{JainKoTh12} first paper on DP-OCO.  
%     \item \cite{SmithTh13} achieve $\sqrt{Td \log^{2.5}(T)}/\diffp$ for pure DP experts (follow the approximate leader with binary tree). 
%     \item \cite[section 5.2]{JainTh14} get $\sqrt{T \log(1/\delta) \log(d)}/\diffp $ for DP experts using FTRL with entropy regularization
%     \item \cite{AgarwalSi17} get $\sqrt{T\log(d)} + \frac{d \log (d) \log^2(T)}{\diffp}$ for pure DP experts using FTRL with Binary tree. Can probably become $\sqrt{d}$ for approximate DP.
%     \item \cite{KairouzMcSoShThXu21} recent DP-OCO. Achieves $\sqrt{d}/T\diffp$ for linear functions (and least squares) and $\sqrt{\sqrt{d}/T\diffp}$ for general convex (for both stochastic and adaptive adversary).
% \end{enumerate}


% %\hac{one pager for now; change later}

\begin{comment}

Differentially Private algorithms for optimization allow learning about the population while ensuring that individual training datum are protected in a strong mathematical sense. Online learning with experts is one of the simplest models for learning from data and unsurprisingly, private algorithms for this problem have been studied for nearly a decade. In this work, we study the fine-grained behavior of the regret of private algorithms in the high-dimensional/high-privacy setting.

We consider the standard full information setting for online learning with experts. There are $d$ experts, and in each round of the game, the algorithm picks an expert $x_t \in [d]$ and nature picks a loss function $l_t : [d] \rightarrow [0,1]$ simultaneously. The algorithm incurs a loss $l_t(x_t)$, and gets to see the full loss function $l_t$. This game is played over $T$ rounds and the (normalized) {\em regret} of the algorithm is defined as \tk{stick to regret rather than to average regret (results are already stated for unnormalized)} \tk{also use $\ell_t$ like in the technical sections}
\[
Reg_T = \frac{1}{T}\sum_{t=1}^T l_t(x_t) - \frac{1}{T} \min_{x^\star \in [d]} \sum_{t=1}^T l_t(x^\star).
\]
The regret thus measures the loss of the algorithm relative to the best single action in hindsight. This setup has formed the basis of our understanding of a large number of algorithms for optimization, including the stochastic gradient descent algorithm commonly used in machine learning. Without privacy constraints, the optimal achievable regret is very well understood and grows as $\Theta(\sqrt{\frac{\log d}{T}})$. \tk{all these bounds should be stated to sum rather than to average}

When optimizing with privacy, we would like the sequence of actions chosen by the algorithm to be differentially private with respect to changing any single loss function $l_t$. This models the setting where each individual user contributes one loss function to the sequence. Differentially private algorithms for online experts have been studied since the work of~\citet{DworkNaPiRo10} who gave an upper bound\footnote{In this introduction, we use $\tilde{O}$ notation to hide logarithmic factors in $T$ and $\frac{1}{\delta}$, when proving $(\eps, \delta)$-DP bounds.} of $\tilde{O}(d/\eps\sqrt{T})$. There has been a sequence of works~\cite{JainKoTh12,SmithTh13,JainTh14,AgarwalSi17} on this problem and the best known bounds scale as $\tilde{O}(\sqrt{\frac{\log d}{T}} + \min(\frac{\sqrt{d}}{\eps T}, \frac{\sqrt{\log d}}{\eps \sqrt{T}})) $.

While for large $\eps$, the privacy term here is dominated by the first non-private term, our goal in this work is to better understand the privacy term, which we do by looking at the setting of small $\eps$. In this case, a more nuanced picture emerges where the power of the adversary has a significant impact on the achievable regret.

In the online learning setup above, while we look at the worst case over nature's choice of the loss function sequence, different models have been studied. In the {\em adaptive adversary} model, nature can choose the loss sequence $\{l_t\}_{t=1}^{T}$ adversarially in an online manner, where the loss $l_t$ can depend arbitrarily on the choices made by the algorithm in previous time steps. A slightly more benign model is the {\em oblivious adversary} model, where nature must pick a sequence of loss functions in advance and this sequence gets revealed to the algorithm one step at a time. While we still take the worst case over all sequences, this adversary is less powerful as the adversary cannot adapt to random choices made by the algorithm. Finally, the {\em stochastic} adversary can only choose a single distribution over loss functions and a fresh sample is drawn from the same distribution at each time step to get $l_t$. Clearly, the adaptive adversary is more powerful than the oblivious one, which in turn is more powerful than the stochastic one. In the non-private learning with experts setting, the best algorithms do equally well against all three classes of adversaries. Typically, these settings start to differ in limited information settings (e.g. the bandit setting).

Somewhat surprisingly, we show that the optimal regret is different for private learning with experts in different settings. In the stochastic adversary setting, we show that a simple algorithm with regret $\tilde{O}(\sqrt{\frac{\log d }{ T}} + \frac{\log d}{\eps T})$ In the oblivious adversary setting, we show a new algorithm that achieves a regret of $\tilde{O}(\sqrt{\frac{\log d }{ T}} + (\frac{\log d}{\eps T})^{2/3})$. For an adaptive adversary, we show that the regret is $\tilde{O}(\sqrt{\frac{\log d }{ T}} + \frac{\sqrt{\log d}}{\eps \sqrt{T}})$, and that the better rate of $\frac{1}{(\eps T)^{2/3}}$ is not achievable.

We show additional results for the ``realizable'' case where the best expert in hindsight has zero loss. 

\end{comment}



==> lower-bounds.tex <==



\section{Lower bounds}
\label{sec:lower-bounds}


In this section, we prove new lower bounds for adaptive adversaries which show a separation from the non-adaptive case. In particular, we show that for $\diffp = 1/\sqrt{T}$, an adaptive adversary can force any \ed-DP algorithm to incur a linear regret $\Omega(T)$. Similarly, any $\diffp$-DP algorithm with $\diffp \le 1/10$ must incur linear regret against adaptive adversaries. 
On the other hand, the results of~\cref{sec:upper-bounds} show that a sub-linear regret is possible for both privacy regimes with oblivious adversaries. 

Our lower bound is based on finger-printing lower bound constructions~\citep{BunUV18} which are the basic technique for proving lower bounds in the offline setting. The following theorem summarizes our main lower bound for \ed-DP. We defer the proof to~\cref{sec:apdx-thm-lb-adaptive-adv}

\begin{theorem}
\label{thm:lb-adaptive-adv}
    Let $T$ be sufficiently large and $d \ge 2 T$.
    Let $\diffp \le 1$ and $\delta \le 1/T^3$.
    If $\A$ is \ed-DP then there is an adaptive adversary such that
    \begin{equation*}
        \E\left[\sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x)\right]
        \ge \Omega \left( \min \left(T, \frac{1}{(\diffp \log T)^2} \right) \right).
    \end{equation*}
\end{theorem}




We also have the following lower bound for pure differential privacy. It shows that pure DP algorithms cannot learn against adaptive adversaries, that is, they must suffer linear regret for constant $\diffp$.
\begin{theorem}
\label{thm:lb-adaptive-adv-pure}
    Let $\diffp \le 1/10$ and $d \ge 2T$.
    If $\A$ is $\diffp$-DP then there is an adaptive adversary such that
    \begin{equation*}
        \E\left[\sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x)\right]
        \ge \Omega \left(T \right).
    \end{equation*}
\end{theorem}



We can also extend the previous lower bounds to larger values of $\diffp$ (see proof in~\cref{sec:thm-lb-large-peps}).
\begin{theorem}
\label{thm:lb-large-peps}
    Let $1 \le k \le O(p^{1-\rho})$ for $0 < \rho < 1$, $d = 2^k \binom{p}{k} = 2^{\Theta(k \log p)}$, $T = p/k$, and $\diffp \le \frac{\sqrt{k/T}}{200 \rho \log(T)}$ where $p$ is sufficiently large. 
    If $\A$ is \ed-DP with $\delta \le 1/T^3$, then there is an adaptive adversary such that
    \begin{equation*}
       \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
        \ge \Omega \left(\frac{\sqrt{T \log d}}{\diffp \log^{3/2} T } \right).
    \end{equation*}
\end{theorem}
% \begin{proof}(sketch)
%     Take an $n \times p$ fingerprinting code with $n = \sqrt{p}$ and design experts for every subset of $k$ columns. Now we need $T = p/k$ rounds to estimate all columns.
% \end{proof}

Finally, we note that for stochastic adversaries, existing lower bounds for DP-SCO immediately imply lower bounds for the online setting using online-to-batch transformations. As there is a lower bound of $\log(d)/T\diffp$ for private selection~\citep{SteinkeUll17b}, this implies a lower bound on the (normalized) excess loss for DP-SCO with linear functions in $\ell_1$-geometry (as one can reduce private selection to this problem; \citealp{AsiFeKoTa21}). This implies a lower bound of $\log(d)/\diffp$ for DP-OPE. 

% \begin{lemma}[\cite{MitzenmacherUp05}, Ch.~4.2.1]
%   \label{lemma:chernoff}
%   Let $X = \sum_{i=1}^n X_i$ for $X_i \simiid \mathsf{Ber}(p)$.
%   Then for $\rho \in [0,1]$,
%   \begin{align*}
%     \P(X > (1+\rho)np ) \le e^{-np\rho^2 /3}.
%   \end{align*}
% \end{lemma}

==> oco-imp.tex <==


\section{Implications for DP-OCO in $\ell_2$-geometry}
\label{sec:oco-imp}
In this section, we derive several implications of our techniques for \emph{differentially private online convex optimization} (DP-OCO) in $\ell_2$-geometry. In this setting, the algorithm chooses $x_t \in \mc{X}$ where $\mc{X} = \{x \in \R^d: \ltwo{x} \le D\}$ and the adversary responds with loss functions $\ell_t: \mc{X} \to \R^d$ that are convex and $L$-Lipschitz. Building on our techniques for DP-OPE, we propose new algorithms that improve over the best existing regret bounds for DP-OCO~\citep{KairouzMcSoShThXu21} which achieve $d^{1/4} \sqrt{T/\diffp}$ for stochastic and adaptive adversaries. Our algorithms obtain (up to logarithmic factors) near-optimal regret $\sqrt{T} + \sqrt{d}/\diffp$ for stochastic adversaries, and $\sqrt{Td} + T^{1/3}d/\diffp$ for adaptive adversaries.


\subsection{Oblivious adversaries}
\label{sec:oco-obl}

Using our private shrinking dartboard algorithm, in this section we develop algorithms that improve the regret for oblivious adversaries. Our algorithms construct a covering of the parameter space $\mc{X}$ then apply our private shrinking dartboard algorithm where the experts are the elements of the cover. By optimizing the size of the cover to balance the error from the approximation error and the error due to the number of experts, we obtain the following regret for DP-OCO in $\ell_2$-geometry. 
We defer the proof to~\cref{sec:apdx-thm-oco-imp}.
\begin{theorem}
\label{sec:thm-oco-imp}
    Let $\mc{X} = \{x \in \R^d: \ltwo{x} \le D\}$ and $\ell_1,\dots,\ell_T : \mc{X} \to \R$ be convex and $L$-Lipschitz functions chosen by an oblivious adversary. 
    There is an
     \ed-DP that has regret
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in \mc{X}} \sum_{t=1}^T \ell_t(x) \right]
        \le LD \cdot O \left( \sqrt{T d \log T } + \frac{T^{1/3} d \log^{1/3}(1/\delta)  \log T}{\diffp} \right)
        .
    \end{equation*}
\end{theorem}

In the high-privacy regime, this result can improve over the previous work~\citep{KairouzMcSoShThXu21} which has regret $\sqrt{T} d^{1/4}/\sqrt{\diffp}$. For example, if $d=1$ and $\diffp = T^{-1/4}$, then our regret is roughly $T^{7/12}$ while their regret is $T^{5/8}$. 


\subsection{Stochastic adversaries}
\label{sec:oco-stoch}
For stochastic adversaries, we use the reduction in~\cref{sec:ub-stoch} (\cref{alg:stoch-adv}) with optimal algorithms for DP-SCO in $\ell_2$-geometry to obtain optimal regret bounds.
More precisely, we use an optimal \ed-DP-SCO algorithm from~\cite{FeldmanKoTa20}, which we call $\Aopt$. As this algorithm has excess loss $\Delta_n = LD \cdot O(1/\sqrt{n} + \sqrt{d}/n\diffp)$, the following result follows immediately from~\cref{thm:ub-stoch-OCO}. We defer the proof to~\cref{sec:apdx-cor-DP-OCO}. 
We also note that we can also obtain regret bounds for pure $\diffp$-DP using existing (pure) DP algorithms for DP-SCO~\citep{AsiLeDu21} with our reduction. 
 
\begin{corollary}[DP-OCO in $\ell_2$-geometry]
\label{cor:DP-OCO}
    Let $\mc{X} = \{ x \in \R^d: \ltwo{x} \le D\}$
    and $\ell_1,\dots,\ell_T : \mc{X} \to \R$ be convex and $L$-Lipschitz functions chosen by a stochastic adversary, $\ell_i \simiid P$.
    %Let $\A$ be an optimal \ed-DP algorithm for DP-SCO with excess loss $O(\Delta_n)$ using $n$ samples. 
    Then
    \cref{alg:stoch-adv} using $\Aopt$ is \ed-DP and has regret
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
        \le LD \cdot O \left(\sqrt{T} + \frac{\sqrt{d} \log T}{\diffp} \right)
    \end{equation*}   
\end{corollary}
This regret is near-optimal up to logarithmic factors since we have the lower bound $\sqrt{T} + \sqrt{d}/\diffp$ for the offline version of this problem (DP-SCO in $\ell_2$-geometry) where all of the samples are given in advance~\citep{BassilySmTh14,BassilyFeTaTh19}.



==> pre.tex <==


\newcommand{\Adv}{\mathsf{Adv}}
\newcommand{\Fl}{\mc{L}} %family of loss functions$

\section{Problem setting and preliminaries}
\label{sec:pre}
{Online prediction from experts} (OPE) is an interactive $T$-round game between an online algorithm $\A$ and adversary $\Adv$. At round $t$, the algorithm $\A$ chooses an expert $x_t \in [d]$ and the adversary $\Adv$ picks a loss function $\ell_t \in \Fl = \{\ell \mid  \ell : [d] \to [0,1]\}$ simultaneously. We let $\A_t(\ell_1,\dots,\ell_{t-1}) = x_t$ denote the mapping of algorithm $\A$ at round $t$. Similarly, we define $\Adv_t$ to be the mapping of the adversary at round $t$ (we provide more details on the input of $\Adv_t$ below depending on the type of the adversary).
The algorithm observes $\ell_t$ (after choosing $x_t$) and incurs loss $\ell_t(x_t)$. For a predefined number of rounds $T$, the regret of the algorithm $\A$ is defined as 
\begin{equation*}
    \reg_T(\A) = \sum_{t=1}^T \ell_t(x_t) - \min_{x^\star \in [d]} \sum_{t=1}^T \ell_t(x^\star).
\end{equation*}
%
%
% In the problem of \emph{online prediction from experts} (OPE), in each round the algorithm chooses an expert $x_t \in [d]$ and nature (adversary) picks a loss function $\ell_t : [d] \to [0,1]$ simultaneously. The algorithm observes $\ell_t$ (after choosing $x_t$) and incurs loss $\ell_t(x_t)$. For a predefined number of rounds $T$, the regret of the algorithm is defined as 
% \begin{equation*}
%     \reg_T = \sum_{t=1}^T \ell_t(x_t) - \min_{x^\star \in [d]} \sum_{t=1}^T \ell_t(x^\star).
% \end{equation*}
%We study two different versions of this problem: the first is \emph{online prediction from experts} (OPE) where $\mc{X} = [d]$ and the loss functions are $\ell_t : [d] \to [0,1]$. The second setting is \emph{online convex optimization} (OCO) in $\ell_2$-geometry \hac{move to one separate section?} where $\mc{X} = \{x \in \R^d: \ltwo{x} \le D\}$ and $\ell_t$ is $L$-Lipschitz. Our main setting of interest in this paper is the former (online experts problem). However, some of the techniques and results that we develop for this problem prove useful for OCO in $\ell_2$-geometry, hence we study the implications of our techniques for this setting as well.
%
We consider three types of adversary $\Adv$ for choosing the sequence of loss functions $\{\ell_t\}_{t=1}^T$. To help define privacy, we will diverge from the traditional presentation of these models in online learning literature. The adversary will consist of a sequence of $T$ data points $z_1,\dots,z_T \in \domain$, and an algorithm $\ell$ that generates the sequence of losses.

For both stochastic and oblivious adversaries the loss function at step $t$ is generated based on data point $z_t$ alone; i.e. $\ell_t(\cdot) = \ell(\cdot; z_t)$, where for all $z \in \domain$, $\ell(\cdot; z)$ is an admissible loss function for the relevant setup. The two models differ in the choice of the sequence $z_1,\ldots,z_T$: for a stochastic adversary, the sequence of $z_i$'s is chosen i.i.d. from some distribution $P$ (chosen by the adversary). For an oblivious adversary, this sequence itself is adversarially chosen. In other words:
\begin{align*}
    Reg_T^{\mbox{(stochastic)}}(\A) &= \sup_{\ell, P} \mathbb{E}_{z_1,\ldots,z_T \sim P^T} [Reg_T(\A) | \ell_t(\cdot) = \ell(\cdot; z_t)],\\
    Reg_T^{\mbox{(oblivious)}}(\A) &= \sup_{\ell} \sup_{z_1,\ldots,z_T \in \domain^T} [Reg_T(\A) | \ell_t(\cdot) = \ell(\cdot; z_t)].
\end{align*}

In the case of an adaptive adversary, the loss at step $t$ can depend on the algorithm's choices in previous steps. Thus $\ell_t(\cdot) = \ell(\cdot; z_t, x_{1:t-1})$, where as before this loss function is constrained to be an admissible loss function for all possible values of inputs $z_t, x_{1:t-1}$. The adaptive regret is then the worst case regret over $z_1,\ldots,Z_T$ and the mapping $\ell$:
\begin{align*}
Reg_T^{\mbox{(adaptive)}}(\A) &= \sup_{\ell} \sup_{z_1,\ldots,z_T \in \domain^T} [Reg_T(\A) | \ell_t(\cdot) = \ell(\cdot; z_t, x_{1:t-1})].
\end{align*}


%We have $T$ data points $z_1,\dots,z_T \in \domain$ such that the adversary at round $t$ uses the $t$'th data point $z_t$ as follows.   \\
%\textbf{Stochastic Adversary:} the loss functions are sampled from a fixed distribution $P$ over $\Fl$. More precisely, $z_t \simiid P$ and  $\Adv_t$ generates a loss function $\ell_t(\cdot) = \Adv_t(z_t) \defeq \ell(\cdot;z_t)$. \\
%\textbf{Oblivious Adversary:} the adversary chooses the sequence of loss functions $(\ell_1,\dots,\ell_T)$ in an arbitrary way before interacting with the algorithm. In particular, there are arbitrary data points $(z_1,\dots,z_T) \in \Fl^T$ such that $\ell_t(\cdot) = \Adv_t(z_t) \defeq \ell(\cdot;z_t)$. \\
%\textbf{Adaptive Adversary:} the adversary chooses the loss function $\ell_t$ at time $t$ after observing the previous decisions of the algorithm $x_1,\dots,x_{t-1}$. More formally, there are data points $(z_1,\dots,z_T) \in \domain^T$ such that $\ell_t(\cdot) = \Adv_t(z_t,x_1,\dots,x_{t-1}) = \ell(\cdot;z_t,x_1,\dots,x_{t-1})$.

Given data $z_{1:T} = (z_1,\dots,z_T) \in \domain^T$, we let $\A \circ \Adv(z_{1:T}) = x_{1:T}$ denote the output of the interaction between the algorithm $\A$ and adversary $\Adv$ given inputs $z_{1:T}$.

Under this setting, the goal is to design private algorithms that minimize the appropriate notion of regret. To this end, we extend the standard definition of \ed-differential privacy~\citep{DworkMcNiSm06,DworkKeMcMiNa06} to the online setting. %Prior work in DP-OPE has mostly focused on privacy against oblivious adversaries~\cite{AgarwalSi17}. 
Like most previous works, we study a stronger notion of privacy that holds even against adaptive adversaries.\footnote{\citet{JainRaSiSm21} recently formalized DP against adaptive adversaries for a different online learning problem. Their notion is equivalent to ours, but our presentation may be easier to work with.} %We begin with DP against oblivious adversary.
%
% \begin{definition}[Oblivious DP~\citealp{AgarwalSi17}]
% \label{def:DP}
% 	A randomized  algorithm $\A$ is \ed-differentially private (\ed-DP) against oblivious adversaries if, for all sequences $\Ds=(z_1,\dots,z_T) \in \domain^T$ and $\Ds'=(z'_1,\dots,z'_T) \in \domain^T$ that differ in a single element, for any oblivious adversary $\Adv$, and for all events $\cO$ in the output space of $\A \circ \Adv$, we have
% 	\[
% 	\Pr[\A \circ \Adv(\Ds)\in \cO] \leq e^{\eps} \Pr[\A \circ \Adv(\Ds')\in \cO] +\delta.
% 	\]
% \end{definition}
%
%We also have the same definition against adaptive adversaries.
\begin{definition}[Adaptive DP]
\label{def:DP}
	A randomized  algorithm $\A$ is \ed-differentially private against adaptive adversaries (\ed-DP) if, for all sequences $\Ds=(z_1,\dots,z_T) \in \domain^T$ and $\Ds'=(z'_1,\dots,z'_T) \in \domain^T$ that differ in a single element, for any $\ell$ defining an adaptive adversary $\Adv$, and for all events $\cO$ in the output space of $\A \circ \Adv$, we have
	\[
	\Pr[\A \circ \Adv(\Ds)\in \cO] \leq e^{\eps} \Pr[\A \circ \Adv(\Ds')\in \cO] +\delta.
	\]
\end{definition}

As remarked earlier, all our algorithms will be differentially private against adaptive adversaries, and the other adversary models are considered only from the the point of view of utility. This is consistent with a long line of work on private learning algorithms, where privacy is proven for worst-case inputs while utility bounds often make distributional or other assumptions on the data.



%Our main problem of interest in this paper is differentially private online prediction from experts (DP-OPE). A related problem which we use in our algorithms is deferentially private stochastic convex optimization (DP-SCO)~\cite{BassilyFeTaTh19}. In this problem, the loss functions are sampled from some distribution $\ell_i \simiid P$ and the goal is to minimize the excess population loss $L(x) = \E_{\ell \sim P}[\ell(x)]$ given $n$ samples $\ell_1,\dots,\ell_n$.

\begin{comment}
\iftoggle{arxiv}{
\subsection{Background on differential privacy}
We recall the following preliminary results on differential privacy which we use throughout the paper.
\begin{lemma}
\label{lemma:adv-comp}
    Let $T \in \N$ and $ \Fl = \{\ell \mid  \ell : [d] \to [0,1]\}$ be the space of loss functions.
    Let $\A_t : \Fl^t \times [d]^{t-1} \to [d]$ be $\diffp_t$-DP. Then for any $\delta>0$, their composition is $(\diffp,\delta)$-DP where
    \begin{equation*}
        \diffp = \frac{3}{2} \sum_{t=1}^T \diffp_t^2 + \sqrt{6 \sum_{t=1}^T \diffp_t^2 \log(1/\delta) }.
    \end{equation*}
\end{lemma}


\newcommand{\AbThr}{AboveThreshold}
\newcommand{\init}{InitializeSparseVec} %initialize an instance with empty set of queries
\newcommand{\addq}{AddQuery} %add a new query
\newcommand{\test}{TestAboThr} % test if last query is above threshold



\subsubsection{Sparse vector technique}
In this section, we recall the sparse-vector-technique~\cite{DworkRo14} which we use for the realizable setting in~\cref{sec:upper-bounds-realizable}. Given an input $\Ds = (z_1,\dots,z_n) \in \domain^n$, the algorithm takes a stream of queries $q_1,q_2,\dots,q_T$ in an online manner. We assume that each $q_i$ is $1$-sensitive, that is, $|q_i(\Ds) - q_i(\Ds') | \le 1$ for neighboring datasets $\Ds,\Ds' \in \domain^n$ that differ in a single element.
We have the following guarantee. 
\begin{lemma}~\cite[theorem 3.24]{DworkRo14}
\label{lemma:svt}
    Let $\Ds = (z_1,\dots,z_n) \in \domain^n$.
    %and $\diffp \le 1$.  
    For a threshold $L$ and $\beta>0$, there is an $\diffp$-DP algorithm (\AbThr) that halts at time $k \in [T+1]$ such that for $\alpha = \frac{8(\log T + \log(2/\beta))}{\diffp}$ with probability at least $1-\beta$
    \begin{itemize}
        \item For all $t < k$, $q_i(\Ds) \le L + \alpha$
        \item $q_k(\Ds) \ge L - \alpha$ or $k = T+1$
    \end{itemize}
\end{lemma}

To facilitate the notation for using \AbThr~in our algorithms, we assume that it has the following components:
\begin{enumerate}
    \item $\init(\diffp,L,\beta)$: initializes a new instance of \AbThr~with privacy parameter $\diffp$, threshold $L$, and probability parameter $\beta$. This returns an instance (data structure) $Q$ that supports the following two functions.
    \item $Q.\addq(q)$: adds a new query $q:\domain^n \to \R$ to $Q$.
    \item $Q.\test()$: tests if the last query that was added to $Q$ was above threshold. In that case, the algorithm stops and does not accept more queries.
\end{enumerate}

% In out algorithm, we will use sparse-vector to identify if the loss of the current expert is large. In particular, at round $t+1$, given $\ell_1,\dots,\ell_{t}$ and previous model $x_{t}$, we define the queries $q_t(\ell_1,\dots,\ell_{t}) = \sum_{j=1}^t \ell_j(x_t)$. Note that $q_t$ is a $1$-sensitive query, and therefore~\Cref{lemma:svt} with $L = 2\alpha$ implies the following result.
% \begin{lemma}~\cite[theorem 3.24]{DworkRo14}
% \label{lemma:svt-OPE}
%     Let $\diffp \le 1$ and $\ell_1,\dots,\ell_T$ be the loss functions in a DP-OPE protocol with corresponding models $x_1,\dots,x_T$.  For $\beta>0$, there is an $\diffp$-DP algorithm (\AbThr) that halts at time $k \in [T+1]$ such that for $\alpha = \frac{8(\log T + \log(2/\beta))}{\diffp}$ with probability at least $1-\beta$
%     \begin{itemize}
%         \item For all $t < k$, $\sum_{j=1}^t \ell_j(x_t) \le 3 \alpha$
%         \item For $t=k$, $\sum_{j=1}^t \ell_j(x_t) \ge \alpha$ or $k = T+1$
%     \end{itemize}
% \end{lemma}

\newcommand{\BinTr}{BinaryTree}

\subsubsection{The binary tree mechanism}
We also build on the binary tree mechanism~\cite{DworkNaPiRo10,ChanShSo11} which allows to privately estimate the running sum of a sequence of $T$ numbers $a_1,\dots,a_T \in [0,1]$.
\begin{lemma}~\cite[theorem 4.1]{DworkNaPiRo10}
\label{lemma:svt}
    Let $\diffp \le 1$.  There is an $\diffp$-DP algorithm (\BinTr) that takes a stream of numbers $a_1,a_2,\dots,a_T$ and outputs $c_1,c_2,\dots,c_T$ such that for all $t \in [T]$ with probability at least $1-\beta$
    \begin{equation*}
        |c_t - \sum_{i=1}^t a_i| \le O \left( \frac{\mathsf{poly}(\log T/\beta)}{\diffp} \right).
    \end{equation*}
\end{lemma}

\paragraph{Notation} For a positive integer $k \in \N$, we let $[k] = \{1,2,\dots,k\}$. Moreover, for $a_1,\dots,a_t$, we let $a_{1:t} = a_1,\dots,a_t$.
}{}

\end{comment}

==> realizable-alg-potential.tex <==

\section{Potential-based algorithm for DP-experts}
\label{sec:alg-pot}
The algorithm in~\cref{alg:SVT-zero-loss} uses the sparse vector technique to evaluate the current arm. In this section, we present a more direct algorithm that uses the sparse vector technique on a potential function. This more direct approach allows us to improve the polylogarithmic terms, which results in significant improvements for DP-OCO as we show in the next section.

We describe the algorithm in a more abstract way, which will translate more easily to OCO. Let $
\mu$ be the uniform measure over the space of experts; this will be the uniform distribution over the finite number of experts in the case of DP-OPE, and the uniform distribution over the unit ball in $\mathbb{R}^d$ in the case of DP-OCO. At a high level, the algorithm is similar to \cref{alg:SVT-zero-loss} in that it samples from the exponential mechanism, and keeps that sample until a certain condition is met. While the condition there dealt only with the chosen expert, we will instead test a global condition. For a parameter $\eta$, we define the potential $\phi_{\eta}(t) = \int \exp(-\eta \sum_{i=1}^t \ell_i(x) \mu(x) \text{d}x$. The condition we check (using the sparse vector technique) is that $\log \phi_{\eta}(t)$ has changed by at least $\alpha$ since the last resample. We formally describe the algorithm in \cref{alg:potential-experts}.


\begin{algorithm}[t]
	\caption{Potential-based Algorithm for Experts}
	\label{alg:potential-experts}
	\begin{algorithmic}[1]
		%\REQUIRE Parameters $\alpha,\bet$
		%constraint set $\xdomain$,
		%step size $\ss$, initial point $x_0$;
		\REQUIRE Switching bound $K$, Parameters $\eta, \alpha$, failure probability $\beta$, per-phase privacy parameter $\diffp_0$, measure $\mu$ on set of experts.
		\STATE Set $k=0$, $t^*(k)=0$ and sample current expert $x_0 \sim \mu$.
  
        \FOR{$t=1$ to $T$\,}
           
            \IF{$k < K$}
                \STATE $Q = \init(\diffp_0,2\alpha,\beta/T)$
                %\STATE Run a new $\AbThr$ instance over the queries $q_t = \sum_{i=1}^{t-1} \ell_i(x_{t-1})$ with privacy parameter $\diffp_0$, probability parameter $\beta/T$, accuracy parameter $\alpha$ and threshold $L=3\alpha$ 
                %\WHILE{$\AbThr$ has not halted}
                \WHILE{Q.\test() = False}
                    \STATE Set $ x_{t} =  x_{t-1}$
                    \STATE Define a new query $q_t = \frac{1}{\eta}(\log \phi_{\eta}(t^*(k)) - \log \phi_{\eta}(t))$
                    \STATE Add new query $Q.\addq(q_t)$
                    \STATE Receive loss function $\ell_t: [d] \to [0,1]$
        	        \STATE Pay cost $\ell_t(x_t)$
        	        \STATE Update $t = t+1$ %and feed a new query $q_t = \sum_{i=1}^{t-1} \ell_i(x_{t-1})$ to \AbThr
                \ENDWHILE
            
                % \STATE Run a Sparse-Vector query to identify if $\sum_{i=1}^{t-1} \ell_i(x_t) \ge \frac{100 \log(d)}{\diffp_0}$
                % \IF{Sparse-Vector identifies above threshold}
                \STATE Sample $x_t$ from the distribution:
                \begin{equation*}
                    P(x_t = x) =  e^{-\eta \sum_{i=1}^{t-1} \ell_i(x) \mu(x)} / \phi_{\eta}(t-1)
                \end{equation*}
                %\STATE Let $ x_{t}$ be the output of the exponential algorithm
                \STATE $k = k + 1$.
                \STATE $t^*(k) = t-1$.
                %\ENDIF
            \ELSE
        	\STATE Set $ x_{t} =  x_{t-1}$
        	\STATE Receive loss function $\ell_t: [d] \to [0,1]$
        	\STATE Pay cost $\ell_t(x_t)$
        	\ENDIF  
        \ENDFOR
	\end{algorithmic}
\end{algorithm}


We first observe some simple properties of $\phi_{\eta}$.
\begin{lemma}
    Suppose that the per-step losses $\ell_t(s)$ are in $[0,1]$. Then $\phi_{\eta}(t-1) \geq \phi_{\eta}(t) \geq e^{-\eta}\phi_{\eta}(t-1)$.
\end{lemma}
\begin{proof}
For any $x$, we have
\begin{align*}
\sum_{i=1}^{t-1} \ell_i(x) \leq  \sum_{i=1}^{t} \ell_i(x) \leq  \sum_{i=1}^{t-1} \ell_i(x) + 1.
\end{align*}
This implies that
\begin{align*}
e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)} \geq e^{-\eta \sum_{i=1}^{t} \ell_i(x)} \geq e^{-\eta} e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)}. 
\end{align*}
The claim follows by integrating with respect to $\mu$.
\end{proof}

\begin{lemma}
\label{lem:svt_worked}
    Suppose that $\alpha \geq \frac{8\eta (\log T + \log 2T/\beta)}{\diffp_0}$. Then during the run of the algorithm, $\log\phi_\eta(t^*(k)) -\log\phi_\eta(t) \leq  3\alpha$ always holds except with probability $\beta$. Moreover, $\log\phi_\eta(t^*(k)) - \log\phi_\eta(t^*(k+1)) \geq \alpha$ holds for all $k$ except with probability $\beta$.    \end{lemma}
\begin{proof}
    We use sparse vector with a threshold of $2\alpha$. The condition on $\alpha$ along with the first property of the sparse vector algorithm~\cref{lemma:svt} implies that if $\log\phi_\eta(t^*) -\log\phi_\eta(t) \leq 3\alpha$. The second property of sparse vector implies the second property.
\end{proof}


We next analyze the loss of the algorithm.
\begin{lemma}
Suppose that $\eta < \frac 1 2$ and losses are in the range $[0,1]$. For some $\gamma > 0$, let $L^*(\gamma)$ be such that $\Pr_{x \sim \mu}[\sum_{t=1}^T \ell_x(t) \leq L^*(\gamma)] \geq \gamma$. Let $K \geq \frac{\eta L^*(\gamma) + \log 1/\gamma}{\alpha}$. Then the expected loss of \cref{alg:potential-experts} satisfies
\begin{align*}
    \E[\sum_{t=1}^T \ell_t(x_t)] \leq 2e^{3\alpha}(L^*(\gamma) + \frac{\log 1/\gamma}{\eta}) + 2\beta T.
\end{align*}
\end{lemma}
\begin{proof}
We first observe that by the assumption on sufficient probability mass on experts with loss at most $L^*(\gamma)$, it follows that $\phi_\eta(T) \geq \gamma e^{-\eta L^*(\gamma)}\phi_\eta(0)$. Let $E$ be the event that both the conditions on $\phi_\eta(t)$'s in ~\cref{lem:svt_worked} hold. Thus $\Pr[E] \geq 1-2\beta$. The second condition implies that if we reach the bound $K$ on the number of switches, then conditioned on $E$, $\phi_\eta(T) \leq e^{-K\alpha}\phi_\eta(0)$. Thus if $K \geq \frac{\eta L^*(\gamma) + \log 1/\gamma}{\alpha}$, then the switching bound is never reached under $E$.

    Now note that if we sampled $x \sim e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)} / \phi_{\eta}(t-1)$, then we would have
    \begin{align*}
        \E[\eta\ell_t(x)/2] &= \frac{1}{\phi_{\eta}(t-1)} \int  \eta\ell_t(x) e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)} \mu(x) \text{d}x\\
        & \leq \frac{1}{\phi_{\eta}(t-1)} \int  (1-e^{-\eta\ell_t(x)})e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)}  \mu(x) \text{d}x\\
        & = \frac{1}{\phi_{\eta}(t-1)} \int (e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)} -  e^{-\eta \sum_{i=1}^{t} \ell_i(x)}) \mu(x) \text{d}x\\
        &= \frac{\phi_{\eta}(t-1)- \phi_{\eta}(t)}{\phi_{\eta}(t-1)}\\
        &\leq \log \frac{\phi_{\eta}(t-1)}{\phi_{\eta}(t)}
    \end{align*}
    Here the first inequality uses the fact that for $y \in [0,1]$, we have $y/2 < 1- e^{-y}$, and the second inequality uses $(1-r) \leq -\log r$ for $r \in [\frac{1}{2},1]$. The assumptions on $\eta$ and the losses imply that the relevant conditions hold.

    Our algorithm however uses an outdated sample based on the distribution at $t^*(k)$, whenever $t$ is in phase $k$. Nevertheless, note that the cumulative losses increase with $t$ so that $e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)}$ is smaller than $e^{-\eta \sum_{i=1}^{t^*(k)} \ell_i(x)}$.% Let $E$ be the event that the ratio $\frac{\phi_{\eta}(t^*(k))}{\phi_{eta}(t-1)} \leq e^{3\alpha}$. Thus $\Pr[E] \geq 1-\beta$. 
    We then write
    \begin{align*}
   \E[\eta\ell_t(x_t)/2 \cdot \mathbf{1}(E)] &= \frac{1}{\phi_{\eta}(t^*(k))} \int  \mathbf{1}(E) \eta\ell_t(x) e^{-\eta \sum_{i=1}^{t^*(k)} \ell_i(x)} \mu(x) \text{d}x\\     &\leq \frac{\phi_{\eta}(t-1)}{\phi_{\eta}(t^*(k))}\cdot  \frac{1}{\phi_{\eta}(t-1)}\int  \eta\ell_t(x) e^{-\eta \sum_{i=1}^{t-1} \ell_i(x)} \mu(x) \text{d}x\\
        &\leq e^{3\alpha}\log \frac{\phi_{\eta}(t-1)}{\phi_{\eta}(t)}.
    \end{align*}
Rearranging and summing over the $t$ steps, we get
    \begin{align*}
   \E[\sum_{t=1}^T\ell_t(x_t)\cdot \mathbf{1}(E)] 
           &\leq \frac{2e^{3\alpha}}{\eta} \sum_{t=1}^T\log \frac{\phi_{\eta}(t-1)}{\phi_{\eta}(t)}\\
           &\leq \frac{2e^{3\alpha}}{\eta} \log \frac{\phi_{\eta}(0)}{\phi_{\eta}(T)}.
    \end{align*}
Since $\phi_\eta(T) \geq \gamma e^{-\eta L^*(\gamma)}\phi_\eta(0)$, we can upper bound this expression.
Furthermore, $\E[\sum_{t=1}^T\ell_t(x_t)\cdot \mathbf{1}(E^c)]$ is clearly bounded $\Pr[E^c] \cdot T \leq 2\beta T$. The claim follows.
\end{proof}

This can yield pure or approximate DP. Indeed each phase of the algorithm satisfies $(\eta + \diffp_0)$-DP. Composing over the at most $K$ phases, we get  $(\eta + \diffp_0)$-DP or $(2(\eta + \diffp_0)\sqrt{K \log 1/\delta}, \delta)$-DP. 
With this in mind, we can now plug in appropriate values of $\eta, \alpha, \eps_0$ to derive the following result for pure $\diffp$-DP.

\begin{theorem}(pure DP)
    Suppose that we run \cref{alg:potential-experts} with parameters $\alpha = 1$, $\beta = \frac{1}{T^2}$,  $K=2 \log 1/\gamma$ , $\diffp_0 = \diffp / K$, and $\eta =\diffp_0 / (56 \log T) = \diffp / (112 \log T \log 1/\gamma)$. If $L^*(\gamma) \leq \log^2 1/\gamma \log T / \diffp$, then this algorithm satisfies $\eps$-DP and incurs loss $O(L^* + \frac{\log^2 1/\gamma\log T}{\diffp})$. In particular, for DP-OPE with $d$ experts, assuming that that $OPT \leq \log^2 d \log T / \diffp$, we get regret  $O(\log^2 d \log T / \diffp)$ by setting $\gamma = \frac 1 d$.
\end{theorem}

Moreover, we have the following improved bound for \ed-DP.
\begin{theorem}(\ed-DP)
\label{thm:pot-appr}
    Suppose that for $\eps < 1$,  we run \cref{alg:potential-experts} with parameters $\alpha = 1$, $\beta = \frac{1}{T^2}$,  $K=2 \log 1/\gamma$ , $\diffp_0 = \diffp / \sqrt{K\log 1/\delta}$, and $\eta =\diffp_0 / (56 \log T) = \diffp / (112 \log T \sqrt{\log 1/\gamma\log 1/\delta})$. If $L^*(\gamma) \leq \log^{1.5} 1/\gamma \log T \sqrt{\log 1/\delta}/ \diffp$, then this algorithm satisfies $(\eps,\delta)$-DP and incurs loss $O(L^* + \frac{\log^{1.5} 1/\gamma\log T\sqrt{\log 1/\delta}}{\diffp})$. In particular, for DP-OPE with $d$ experts, assuming that $OPT \leq \log^{1.5} d \log T\sqrt{\log 1/\delta} / \diffp$, we get regret  $O(\log^{1.5} d \log T \sqrt{\log 1/\delta}/ \diffp)$ by setting $\gamma = \frac 1 d$.
\end{theorem}


For the setting of DP-OCO in the realizable case, we get that by Lipschitzness, a small ball of radius $r$ around $x^*$ has loss $O(rLT)$. Setting $r=(LT)^{-1}$ then ensures that this value is at most $1$ This ball has measure $\gamma = (r/D)^{-d}$. Scaling so that $D,L \leq 1$, 
{we get an regret $O(d^2 \log^3 T / \diffp)$ for the case of $\eps$-DP and $O(d^{1.5}\log^{2.5}  T \sqrt{\log 1/\delta}/ \diffp)$ for $(\eps,\delta)$-DP.} Finally we note that this algorithm only accesses the loss functions to sample from the exponential mechanism, and compute the potential $\phi_{\eta}(t)$. Both of these can be implemented in polynomial time for the case of $\mu$ being uniform over the ball, and the losses being convex using standard techniques from logconcave sampling. Thus this algorithm can be run in polynomial time for DP-OCO.


==> upper-bounds.tex <==


\section{Private algorithms for prediction from experts}
\label{sec:upper-bounds}
We begin our algorithmic contribution by developing new algorithms for oblivious (\cref{sec:ub-obl-sd}) and stochastic adversaries (\cref{sec:ub-stoch}). %We develop algorithms for stochastic adversaries (\cref{sec:ub-stoch}), oblivious adversaries (\cref{sec:ub-obl-sd}), and adaptive adversaries (\cref{sec:adap-adv}). 
The main idea is to save the privacy budget by limiting the number of model updates. Though, the way in which this is done varies significantly depending on the adversary: for stochastic adversaries, we allow for $\log(T)$ updates at fixed time-steps $t=2^i$, while for oblivious adversaries we employ a more adaptive time-step strategy for updates based on the underlying data.





\begin{comment}

The following theorem summarizes the guarantees of~\cref{alg:stoch-adv}. For simplicity, we only state the result for the private experts setting, however, we note that a more general statement holds for general convex functions.
\begin{theorem}
\label{thm:ub-stoch}
    Let $\ell_1,\dots,\ell_T \in [0,1]^d$ be chosen by a stochastic adversary, $\ell_i \simiid P$. \cref{alg:stoch-adv} is \ed-DP and has regret
    \begin{equation*}
        \E_{\ell_t \sim P} \left[\ell_t(x_t) - \min_{x \in [d]} \ell_t(x) \right] \le O \left( \sqrt{\frac{\log(d)}{2^i}} +  \frac{\log(d)}{2^i \diffp} \right).
    \end{equation*}
    Therefore at phase $i$, that is $2^{i} \le t \le 2^{i+1}$, the total regret is at most 
    \begin{equation*}
    \E\left[ \sum_{t=2^{i}}^{2^{i+1}}\ell_t(x_t) - \min_{x \in [d]} \sum_{t=2^{i}}^{2^{i+1}} \ell_t(x) \right] 
        \le O \left(\sqrt{2^i \log(d)} + \frac{\log(d)}{ \diffp}\right).
    \end{equation*}
\end{theorem}

\begin{proof}
    The privacy claim is immediate as each sample $\ell_i$ is used only once in running a single \ed-DP algorithm. Now we prove the claim about utility. Consider time-step $t=2^i$ where we invoke a DP-SCO algorithm with $t/2 = 2^{i-1}$ samples. Therefore the guarantees of such algorithms~\cite[theorem 6]{AsiFeKoTa21} imply that at iteration $t$ we have
    \begin{equation*}
        \E_{\ell_t \sim P} \left[\ell_t(x_t) - \min_{x \in [d]} \ell_t(x) \right] \le O \left( \sqrt{\frac{\log(d)}{2^i}} +  \frac{\log(d)}{2^i \diffp} \right).
    \end{equation*}
    Therefore at phase $i$, that is $2^{i} \le t \le 2^{i+1}$, the total regret is at most 
    \begin{equation*}
    \E\left[ \sum_{t=2^{i}}^{2^{i+1}}\ell_t(x_t) - \min_{x \in [d]} \sum_{t=2^{i}}^{2^{i+1}} \ell_t(x) \right] 
        \le O \left(\sqrt{2^i \log(d)} + \frac{\log(d)}{ \diffp}\right).
    \end{equation*}
    As we have at most $\log(n)$ phases with $1 \le i \le \log(T)$, the total regret of~\cref{alg:stoch-adv} is at most $O(\sqrt{T\log (d)} + {\log(d) \log(T)}/{ \diffp})$ which proves the claim.
\end{proof}
\end{comment}


\begin{comment}

\subsection{Oblivious adversaries}
\label{sec:ub-obl}
In this section we consider the stronger model of oblivious adversaries and develop an algorithm with regret $O(\sqrt{T} + T^{1/3}/\diffp^{2/3})$ in this setting. Our algorithm builds on follow-the-lazy-leader where we identify update-steps using sparse-vector-technique. We provide full details in~\cref{alg:obl-adv}. \\

\hac{TODO: need to figure out proof details.}


\begin{algorithm}
	\caption{Follow-the-lazy-leader with sparse-vector}
	\label{alg:obl-adv}
	\begin{algorithmic}[1]
	    \REQUIRE Noise parameter $\Delta > 0$, switching budget $K$
		\STATE Set $x_0 = 1$
		\STATE Set $\diffp_i = \diffp/\sqrt{K}$ and $k=0$
		\STATE Sample $p_0 \sim \lap(\Delta)^d$
        \FOR{$t=1$ to $T$\,}
            \STATE $x_t = x_{t-1}$
            \STATE Define queries $q_x(\ell_{1:t-1}) = p_0(x_t) - p_0(x) + \sum_{i=1}^{t-1} \ell_i(x_t) - \ell_i(x)$ for $x \in [d]$
            \STATE Use Sparse-Vec-tech with $\diffp_i$ privacy to identify if $q_x(\ell_{1:t-1}) > -\Delta/10$ for $x \neq x_t$ \hac{formalize}
            %$p_0(x_t) + \sum_{i=1}^{t-1} \ell_i(x_t) < p_0(x) + \sum_{i=1}^{t-1} \ell_i(x) - 2/\diffp$ for all other $x \in [d]$
            \IF{$k<K$ and Sparse-Vec identifies above thershold}
                \STATE Sample new   $p_0 \sim \lap(\Delta)^d$
                \STATE $x_t = \argmin_{x \in [d]} p_0(x) + \sum_{i=1}^{t-1} \ell_i(x) $
                \STATE $k = k + 1$
            \ENDIF
            \STATE Receive $\ell_t \in \R^d$
            \STATE Pay cost $\ell_t(x_t)$
            %\STATE $t = t + 1$
        \ENDFOR
	\end{algorithmic}
\end{algorithm}

The following theorem shows our improved upper bound for oblivious adversaries.
\begin{theorem}
\label{thm:ub-obl}
    Let $\ell_1,\dots,\ell_T \in [0,1]^d$ be chosen by an oblivious adversary. \cref{alg:obl-adv} with $\Delta = T^{1/3}/\diffp^{2/3}$ is \ed-DP and has regret
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
        \le O \left(\sqrt{T\log(d)} +  \frac{ T^{1/3} \log(d)}{\diffp^{2/3}} \right).
    \end{equation*}
\end{theorem}

\begin{proof}
    The privacy proof follows from the guarantees for sparse-vector and the report-noisy-max mechanisms. \hac{formalize more}
    
    The utility proof has two main steps.  In the first step, we analyze the same procedure while allowing $x_t$ to depend on $\ell_t$, that is, we analyze the regret of $\bar x_t = \argmin_{x \in [d]} p_0(x) + \sum_{i=1}^{t} \ell_i(x) $ and show the desired upper bound. In the second step, we show that the regret of the original algorithm is not different from the procedure of step $1$. Let us denote $M(v) = \argmin_{x \in [d]} v(x)$ for $v: [d] \to [0,1]$. The proof will follow directly from the following two lemmas.
    \begin{lemma}
    \label{lemma:step-one}
    For $\diffp \le 1/T^{1/4}$, we have
    \begin{equation*}
     \E \left[ \sum_{t=1}^T \<\bar x_t,\ell_t\> - \min_{x\opt \in[d]} \sum_{t=1}^T \<x\opt,\ell_t\>  \right]
        \le O(\Delta).
    \end{equation*}
    \end{lemma}
    
    \begin{lemma}
    \label{lemma:step-two}
    For $\diffp \le 1/T^{1/4}$, we have
    \begin{equation*}
     \E \left[\sum_{t=1}^T \<x_t - \bar x_t, \ell_t\> \right] 
        \le O(\sqrt{T}).
    \end{equation*}
    \end{lemma}
    The choice of  $\Delta = T^{1/3}/\diffp^{2/3}$ now implies the claim. 
\end{proof}

Now we proceed to prove Lemmas~\ref{lemma:step-one} and~\ref{lemma:step-two}.
\begin{proof}(\cref{lemma:step-two})
    %We start with the proof of the second step as it is simpler.
    We will show that each $x_t$ is $(1/\sqrt{T},\delta)$-DP. To this end, we can view the algorithm as a sequence of applications of the 1-AboveThreshold algorithm and then an application of the Laplace mechanism where each such phase---application of AboveThreshold and Lapalce---is $\diffp_i$-DP. As $x_t$ is a subset of the output of one phase, it is also $\diffp_i$-DP. \hac{formalize}
    %Using this view, we can describe the output of the algorithm as $(t_1,t_2,\dots,t_K)$ and $x_{t_1},x_{t_2},\dots,x_{t_K}$.
    %The properties of 1-AboveThreshold and the Laplace mechanism imply that each $x_{t_i}$ is $\diffp_i$-DP. As $x_t = x_{t_i}$ for some $t_i \le t$, we get that $x_t$ is also $\diffp_i$-DP.
    Recalling that $x_t = M(p_\ell + \sum_{i=1}^{t-1} \ell_i)$ and $\bar x_t = M(p_\ell + \sum_{i=1}^{t} \ell_i)$ \hac{need to say something about $k<K$ whp here}, this now implies that $x_t$ and $\bar x_t$ are $(\frac{1}{\sqrt{T}},\delta)$-indistinguishable. Therefore we have
    \begin{align*}
    \E \left[\sum_{t=1}^T \<x_t - \bar x_t, \ell_t\> \right] 
        & \le \sum_{t=1}^T \lone{ \E x_t - \E \bar x_t} \\
        & \le \sum_{t=1}^T \lone{ \sum_{j=1}^d (P(x_t = e_j) - P(\bar x_t = e_j) ) e_j } \\
        & \le \sum_{t=1}^T  \sum_{j=1}^d \left|P(x_t = e_j) - \delta +  P(\bar x_t = e_j)\right|  + \delta T d \\
        & \le \sum_{t=1}^T \sum_{j=1}^d  \left| P(\bar x_t = e_j) (\frac{P( x_t = e_j) - \delta}{P(\bar x_t = e_j)} - 1) \right| + \delta T d\\
         & \le \sum_{t=1}^T  \sum_{j=1}^d \left| P(\bar x_t = e_j) (e^\diffp - 1) \right| + \delta T d \\
        & \le T (e^\diffp - 1) + \delta T d 
           \le  O(\sqrt{T}).
    \end{align*}    
\end{proof}
    
\begin{proof}(\cref{lemma:step-one})
    %Let us now proceed to the first step. 
    %Let $k$ denote the number of switches of the algorithm and 
    Let $t_1<t_2<\dots <t_K$ denote the switching times. We can show that with high probability $K \le O((T \diffp)^{2/3}) \le \sqrt{T}$ as we assume without loss of generality that $\diffp \le 1/T^{1/4}$. We will upper bound the regret after conditioning on the switching times $(t_1,\dots,t_k)$. First, note that using Be-The-Leader lemma (Lemma 3.1 in \cite{KalaiVe05}) we have
    \begin{align*}
    \sum_{t=1}^T \<\bar x_t,\ell_t\>
        & = \sum_{t=1}^T \<M(p_\ell + \sum_{i=1}^{t} \ell_i),\ell_t\> \\
        & \le \sum_{t=1}^T \<M( \sum_{i=1}^{T} \ell_i),\ell_t\>
            + \sum_{t=1}^T \|p_{t+1} - p_t\|_{\infty},
    \end{align*}
    which implies the regret is upper bounded by
     \begin{align*}
    \sum_{t=1}^T \<\bar x_t,\ell_t\> - \min_{x\opt \in[d]} \sum_{t=1}^T \<x\opt,\ell_t\> 
        \le \sum_{t=1}^T \|p_{t+1} - p_t\|_{\infty},
    \end{align*}
    We will upper bound the expected regret by conditioning first on $(t_1,\dots,t_K)$. Note that we will have $p_0,p_1,\dots,p_{K+1}$ and the regret is upper bounded by 
    \begin{align*}
    \E \left[ \sum_{t=1}^T \|p_{t+1} - p_t\|_{\infty} \mid t_1,t_2,\dots,t_K \right] 
        & \le \sum_{j=1}^K \E \left[ \|p_{j+1} - p_j\|_{\infty} \mid  t_1,t_2,\dots,t_K \right] \\
        & = \sum_{j=1}^K \E \left[ \|p_{j+1} - p_j\|_{\infty} \mid  t_j,t_{j+1},t_{j+2} \right],
    \end{align*}
    where the equality follows since each $p_j$ is independent of $t_{j'}$ for $j' < j$ or $j' > j+1$ \hac{prove this?}. 
    We have two observations that allow to upper bound this quantity. First, without any conditioning, $p_{j+1}$ and $p_j$ have the same distribution. Secondly, the switching times $(t_j,t_{j+1},t_{j+2})$ are $O(1/\sqrt{T})$-DP. We can show that \hac{show this: something not quite right here..}
    \begin{equation*}
     \E \left[ \|p_{j+1} - p_j\|_{\infty} \mid  t_j,t_{j+1},t_{j+2} \right]
        \le O\left( \frac{\linf{p_j + p_{j+1}}}{\sqrt{T}} \right)
        \le O\left( \frac{\Delta}{\sqrt{T}} \right).
    \end{equation*}
    Overall as $K \le O(\sqrt{T} \log(T))$ we get that
    \begin{equation*}
     \E \left[ \sum_{t=1}^T \|p_{t+1} - p_t\|_{\infty} \mid t_1,t_2,\dots,t_K \right] 
        \le O\left( K \frac{\Delta}{\sqrt{T}} \right)
        \le O(\Delta).
    \end{equation*}
    The law of iterated expectation now gives the claim.
\end{proof}


\begin{lemma}
\label{lemma:limited-switches}
    Let $\diffp \le 1/T^{1/4}$. For $\Delta \ge T^{1/3}/\diffp^{2/3}$ and $K = \sqrt{T} \log(T)$,
    \begin{equation*}
        P(k \ge K) \le 1/T^{10}.
    \end{equation*}
\end{lemma}
\begin{proof}
    \hac{complete}
    
    Idea: we define a good switch and a bad switch. A good switch is one that has a sequence of size at least $\Delta$. We will show that each sequence is good with constant probability. This implies that the number of good and bad switches is roughly $T/\Delta = (T\diffp)^{2/3} \le \sqrt{T}$.
    
    What is expected length of a sequence?
    
\end{proof}


Ideas for analysis: 
\begin{itemize}
    \item Important: we will analyze the algorithm for $\diffp \le 1/T^{1/4}$ as we can get regret $\sqrt{T}$ for such $\diffp$.
    \item We will have $k = O((T \diffp)^{2/3}) \le O(\sqrt{T})$ switches whp.
    \item Let $t_1<t_2<\dots<t_k$ denote the switching times with noise vectors $p_1,p_2,\dots,p_k \in \R^d$.
    \item We can write in phase $\ell$ for $t_{\ell-1}<t<t_\ell$
    \begin{equation*}
        x_t = \argmin_{x \in [d]} p_\ell(x) + \sum_{i=1}^{t-1} \ell_i(x)
    \end{equation*}
    \item We will have two types of error in the regret:
    \begin{enumerate}
        \item Error from changing $p_i$: as we have at most $k=O(\sqrt{T})$ switches, this will result in error $k |p_{t_2} - p_{t_1}|$. We have to show that $|p_{t_2} - p_{t_1}| = O(1)$.
        \item Error for difference between follow the leader and follow the previous leader. For this, we use the fact that each iterate $x_t$ is $O(1/\sqrt{T})$-DP for $\diffp \le 1/T^{1/4}$ which will imply an error of $O(1/\sqrt{T})$ for each round, that is, error $O(\sqrt{T})$ for the final regret.
    \end{enumerate}
\end{itemize}

\end{comment}


\subsection{Oblivious adversaries using shrinking dartboard}
\label{sec:ub-obl-sd}
In this section, we present our main algorithms for DP-OPE with oblivious adversaries. We build on the shrinking dartboard algorithm~\citep{GeulenVoWi10} to develop a private algorithm that improves over the best existing results for both pure and approximate DP. For $\diffp$-DP, our algorithm obtains regret $\diffp^{-1} \sqrt{T} \log d$ which nearly matches the non-private regret for constant $\diffp$; this is the first algorithm for pure DP that achieves sub-linear regret for oblivious adversaries. For approximate DP, our algorithm obtains regret $\sqrt{T \log d } + \diffp^{-1} (T\log(1/\delta))^{1/3} \log d$: our algorithm achieves negligible privacy cost compared to the non-private regret in the high-dimensional regime. Previous algorithms  obtain regret roughly $\diffp^{-1} \sqrt{T \log d \log(1/\delta)}$ for $d \ge T$ which is $\diffp^{-1} \sqrt{\log(1/\delta)}$ larger than the non-private regret.  

Key to our improvements in this section (similarly to limited switching OPE; \citealp{GeulenVoWi10}) is the observation that the distribution of the multiplicative weights (MW) algorithm does not change significantly between consecutive time-steps. Thus, by using a correlated sampling procedure, we can preserve the same marginal distribution as MW while updating the model with small probability. As this limits the number of model updates, this will allow us to assign higher privacy budget for each model update, hence improving its utility.

Another obstacle that arises from this approach is that the switching probability (to preserve the same marginal distribution) depends on the underlying data $p_{\mathsf{switch}} = 1 - (1-\eta)^{\ell_{t-1}(x_{t-1})}$. This is clearly not private as the probability of switching is zero whenever $\ell_{t-1}(x_{t-1})=0$. To tackle this issue, we guarantee privacy by adding another switching step that forces the algorithm to switch with probability $p$ regardless of the underlying data.


\begin{algorithm}
	\caption{Private Shrinking Dartboard}
	\label{alg:SD}
	\begin{algorithmic}[1]
	    \REQUIRE Step size $\eta > 0$, switching probability $p \in [0,1]$, switching budget $K$
		\STATE Set $w^1_i = 1$, $p^1_i = \frac{1}{d}$ for all $i \in [d]$
		\STATE Choose expert $x_1$ from the distribution $P^1 = (p^1_1,\dots,p^1_d)$
		\STATE Set $k = 1$
        \FOR{$t=2$ to $T$\,}
            \STATE Set $w^t_i = w^{t-1}_i (1 - \eta)^{\ell_{t-1}(i)}$ for all $i \in [d]$
            \STATE Set $p^t_i = \frac{w^t_i}{\sum_{i'=1}^d w^t_{i'}}$ for all $i \in [d]$
            \STATE Sample $z_t \sim \mathsf{Ber}(1-p)$
            \IF{$z_t=1$}
            \STATE Sample $z_t \sim \mathsf{Ber}(w^t_{x_{t-1}}/w^{t-1}_{x_{t-1}})$
            \ENDIF
            % \STATE \hac{maybe this:} Sample from
            % \begin{equation*}
            %     z_t \sim 
            %     \begin{cases}
            %         & \mathsf{Ber}(1-\eta) \quad \quad \quad  \text{   if } \ell_{t-1}(x_{t-1}) = 1 \\
            %         & \mathsf{Ber}(1-\eta) \quad \quad \quad  \text{   if } \ell_{t-1}(x_{t-1}) = 0 \\        
            %     \end{cases}
            % \end{equation*}
            \IF{$z_t = 1$}
                \STATE $x_t = x_{t-1}$
            \ELSIF{$k < K$}
                \STATE $k = k + 1$
                \STATE Sample $x_t$ from $P^t$
            \ENDIF
            \STATE Receive $\ell_t: [d] \to [0,1]$
            \STATE Pay cost $\ell_t(x_t)$
        \ENDFOR
	\end{algorithmic}
\end{algorithm}

The following theorem states the privacy guarantees and the upper bounds on the regret of~\cref{alg:SD}. We defer the proof to~\cref{sec:proof-thm-ub-DS}.
\begin{theorem}
\label{thm:ub-priv-DS}
    %Let $\diffp \le \sqrt{\log d}/T^{1/6}$ and $\delta \le 1$.
    Let $\ell_1,\dots,\ell_T \in [0,1]^d$ be chosen by an oblivious adversary. \cref{alg:SD} with $p < 1/2$, $\eta<1/2$, and $K = 4 T p $ has regret
    %$p = 1/T^{1/3} < 1/2$, $\eta = p \diffp$, and $K =2 T p $ is $(\diffp_f,\delta)$-DP where $\diffp_f = $ and has regret
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
        \le \eta T
        + \frac{\ln d}{\eta} + 2 T e^{-Tp/3}.
        %\left(  \frac{\sqrt{T}}{\diffp} \right)^{2/3} \log d \right).
    \end{equation*}
    Moreover, \cref{alg:SD} is $(\diffp,\delta)$-DP where 
    \begin{equation*}
     \diffp = 
     \begin{cases}
         \frac{5\eta}{p} + 100 T p  \eta^2 + 20 \eta \sqrt{ T p \log(1/\delta)} & \text{if } \delta>0 ;\\
         \frac{\eta}{p} + 16 T p \eta & \text{if } \delta = 0 .
     \end{cases}
    \end{equation*}
\end{theorem}

\iftoggle{arxiv}{
Before proving~\cref{thm:ub-priv-DS}, we illustrate the implication of this result when optimizing the parameters in the algorithm. We have the following regret for approximate DP (see~\cref{sec:apdx-cor-sd-appr} for the proof).}
{
We illustrate the implication of this result when optimizing the parameters in the algorithm. We have the following regret for approximate DP (see~\cref{sec:apdx-cor-sd-appr} for the proof).
}
\begin{corollary}
\label{cor:sd-appr}
    Let $\ell_1,\dots,\ell_T \in [0,1]^d$ be chosen by an oblivious adversary.
    Let $\diffp \le 1$ and set $\diffp_0 = \min(\diffp/2, \log^{1/3}(1/\delta) T^{-1/6} \sqrt{\ln d})$ and $0 < \delta \le 1$ such that $T \ge \Omega(\log(1/\delta))$.  Setting $p = 1/(T \log(1/\delta))^{1/3}$ and $\eta = p \diffp_0/20$, \cref{alg:SD} is \ed-DP and has regret 
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
     \le O \left( \sqrt{T \ln d } + \frac{T^{1/3} \log^{1/3}(1/\delta) \ln d}{\diffp}  \right).
    \end{equation*}
\end{corollary}
% \begin{proof}
%     For these parameters, \cref{alg:SD} has privacy
%     \begin{equation*}
%     \diffp/2 +  T p^3 \diffp^2/10 +  \diffp  \sqrt{12 T p^3\log(1/\delta)} \le \diffp.
%     \end{equation*}
%     Moreover, its regret is
%     \begin{align*}
%      \eta T
%         + \frac{\ln d}{\eta} + 2 T e^{-Tp/3} 
%     & \le T p \diffp/10 + 10 \ln d /(p\diffp) + 2 T e^{-Tp/3} \\
%     & \le \frac{T^{2/3} \diffp}{\log^{1/3}(1/\delta)} + \frac{T^{1/3} \log^{1/3}(1/\delta) \ln d}{\diffp} + 2 T e^{-Tp/3} \\
%     & \le \sqrt{T \ln d } + \frac{T^{1/3} \log^{1/3}(1/\delta) \ln d}{\diffp} + 2 T e^{-Tp/3},
%     \end{align*}
%     where the last inequality follows by taking $\diffp \le \frac{\log^{1/3}(1/\delta) \sqrt{\ln d}}{T^{1/6}}$.
% \end{proof}
Moreover, we have the following regret for pure DP (proof in~\cref{sec:apdx-cor-pure}).
\begin{corollary}
\label{cor:pure}
    Let $\ell_1,\dots,\ell_T \in [0,1]^d$ be chosen by an oblivious adversary.
    Let $\diffp \le 1$. Setting $p = 1/\sqrt{T}$ and $\eta = p \diffp/20$, \cref{alg:SD} is $\diffp$-DP and has regret 
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
     \le O \left( \frac{\sqrt{T} \ln d}{\diffp}  \right).
    \end{equation*}
\end{corollary}
% \begin{proof}
%     For these parameters, \cref{alg:SD} has privacy
%     \begin{equation*}
%     \diffp/10 +  2 Tp \eta 
%     \le \diffp/10 +  Tp^2 \diffp/5
%     \le \diffp.
%     \end{equation*}
%     Moreover, its regret is
%     \begin{align*}
%      \eta T
%         + \frac{\ln d}{\eta} + 2 T e^{-Tp/3} 
%     & \le T p \diffp/10 + 10 \ln d /(p\diffp) + 2 T e^{-Tp/3} \\
%     & \le \sqrt{T \ln d} + \frac{\sqrt{T} \ln d}{\diffp} + 2 T e^{-Tp/3},
%     \end{align*}
%     where the last inequality follows since $\diffp \le 1$.
% \end{proof}


\subsubsection{Private batched shrinking dartboard}
For smaller values of $\diffp$, we present a batch version of~\cref{alg:SD} that groups losses in a batch of size $B$ and applies the same update. 
For a batch size $B$, we define the grouped loss
\begin{equation*}
    \tilde \ell_t = \frac{1}{B} \sum_{i=Bt}^{B(t+1)} \ell_i.
\end{equation*}
The batch version of~\cref{alg:SD} then runs~\cref{alg:SD} on the grouped loss $\tilde \ell_t $ for $\tilde T = \ceil{T/B}$ iterations.
\iftoggle{arxiv}{%
The following theorem state the regret of this algorithm. We prove the theorem in~\cref{sec:apdx-thm-ub-priv-DS-batch}
\begin{theorem}
\label{thm:ub-priv-DS-batch}
    %Let $\diffp \le \sqrt{\log d}/T^{1/6}$ and $\delta \le 1$.
    Let $\ell_1,\dots,\ell_T \in [0,1]^d$ be chosen by an oblivious adversary. \cref{alg:SD} with batch size $1 \le B \le T$, $p < 1/2$, $\eta<1/2$, and $K = 4 T p/B $ has regret
    %$p = 1/T^{1/3} < 1/2$, $\eta = p \diffp$, and $K =2 T p $ is $(\diffp_f,\delta)$-DP where $\diffp_f = $ and has regret
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
        \le \eta T
        + \frac{B \ln d}{\eta} + 2 T e^{-Tp/3B}.
        %\left(  \frac{\sqrt{T}}{\diffp} \right)^{2/3} \log d \right).
    \end{equation*}
    Moreover, for $\delta>0$, \cref{alg:SD} is $(\diffp,\delta)$-DP where 
    \begin{equation*}
     \diffp = 
          \frac{5\eta}{Bp} + 100 T p  \eta^2/B^3 + \frac{20\eta}{B} \sqrt{12 T p/B \log(1/\delta)}
          . 
    \end{equation*}
\end{theorem}
Optimizing the batch size $B$, we obtain the following regret. \cref{fig:comp} illustrates that this algorithm offers improvements over the original version (without batches) in the high-privacy regime. We defer the proof to~\cref{sec:adpx-cor-sd-batch}.
\begin{corollary}
\label{cor:sd-batch}
    Let $\frac{\log^{2/3}(1/\delta) \log(d)}{T} \le \diffp \le \frac{\log^{2/3}(1/\delta) \log(d)}{T^{1/3}} $ and $\delta \le 1$. Setting $B = \frac{\log^{2/5}(1/\delta) \log^{3/5}(d)}{T^{1/5} \diffp^{3/5}} $, $p = (\frac{B}{T \log(1/\delta)})^{1/3}$ and $\eta = B p \diffp/40$, \cref{alg:SD} is \ed-DP and has regret 
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
     \le O \left( \frac{T^{2/5} \log^{1/5}(1/\delta) \log^{4/5}(d))  }{\diffp^{4/5}}  + 2 T e^{-Tp/3B} \right).
    \end{equation*}
\end{corollary}}
{
Following similar steps as in the previous section, we obtain the following regret bounds for this algorithm (proof in~\cref{sec:adpx-cor-sd-batch}). \cref{fig:comp} illustrates that this algorithm offers improvements over the original version (without batches) in the high-privacy regime.
\begin{theorem}
\label{cor:sd-batch}
    Let $\frac{\log^{2/3}(1/\delta) \log(d)}{T} \le \diffp \le \frac{\log^{2/3}(1/\delta) \log(d)}{T^{1/3}} $ and $\delta \le 1$. Setting $B = \frac{\log^{2/5}(1/\delta) \log^{3/5}(d)}{T^{1/5} \diffp^{3/5}} $, $p = (\frac{B}{T \log(1/\delta)})^{1/3}$ and $\eta = B p \diffp/40$, \cref{alg:SD} is \ed-DP and has regret 
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
     \le O \left( \frac{T^{2/5} \log^{1/5}(1/\delta) \log^{4/5}(d))  }{\diffp^{4/5}}  + 2 T e^{-Tp/3B} \right).
    \end{equation*}
\end{theorem}
}
% \begin{proof}
%     For these parameters, \cref{alg:SD} has privacy
%     \begin{equation*}
%     \frac{5\eta}{Bp} + \frac{4 T p  \eta^2}{B^3} + \frac{\eta}{B^{3/2}} \sqrt{12 T p \log(1/\delta)} = O(\diffp).
%     \end{equation*}
%     Moreover, its regret is
%     \begin{align*}
%      \eta T
%         + \frac{B\ln d}{\eta} + 2 T e^{-Tp/3B} 
%     & \le T B p \diffp/10 + 10 \ln d /(p\diffp) + 2 T e^{-Tp/3B} \\
%     & \le \frac{T^{2/3} B^{4/3} \diffp}{\log^{1/3}(1/\delta)} + \frac{T^{1/3} \log^{1/3}(1/\delta) \ln d}{B^{1/3}\diffp} + 2 T e^{-Tp/3B} \\
%     & \le \frac{T^{2/5} \log^{1/5}(1/\delta) \log^{4/5}(d))  }{\diffp^{4/5}}  + 2 T e^{-Tp/3B},
%     \end{align*}
%     where the last inequality follows by choosing $B = \frac{\log^{2/5}(1/\delta) \log^{3/5}(d)}{T^{1/5} \diffp^{3/5}} $ (note that $B \ge 1$ for $\diffp \le  \frac{\log^{2/3}(1/\delta) \log(d)}{T^{1/3}}$) and noticing that $Tp/B \ge \Omega(T)$ as we have a lower bound on $\diffp$. \hac{do this calculation again} %$\diffp \le \frac{\log^{1/3}(1/\delta) \sqrt{\ln d}}{T^{1/6} B^{5/6}}$.
% \end{proof}

\begin{comment}
\subsubsection{Implications for DP-OCO over the sphere}
\label{sec:imp-oco}
Building on our upper bounds for private prediction from experts, in this section we develop algorithms that improve over the best existing bounds for DP-OCO in $\ell_2$-geometry. Our algorithms construct a covering of the parameter space then apply our private shrinking dartboard algorithm over this cover. By optimizing the size of the cover to balance the error from the approximation error and the error due to the dimensionality, we obtain the following regret for DP-OCO in $\ell_2$-geometry. 
We defer the proof to~\cref{sec:apdx-thm-oco-imp}.
\begin{theorem}
\label{sec:thm-oco-imp}
    Let $\mc{X} = \{x \in \R^d: \ltwo{x} \le D\}$ and $\ell_1,\dots,\ell_T : \mc{X} \to \R$ be convex and $L$-Lipschitz functions chosen by an oblivious adversary. 
    There is an
     \ed-DP that has regret
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in \mc{X}} \sum_{t=1}^T \ell_t(x) \right]
        \le LD \cdot O \left( \sqrt{T d \log T } + \frac{T^{1/3} d \log^{1/3}(1/\delta)  \log T}{\diffp} \right)
    \end{equation*}
\end{theorem}

In the high-privacy regime, this result can improve over the previous work~\cite{KairouzMcSoShThXu21} which has regret $\sqrt{T} d^{1/4}/\sqrt{\diffp}$. For example, if $d=1$ and $\diffp = T^{-1/4}$, then our regret is roughly $T^{7/12}$ while their regret is $T^{5/8}$. \hac{modify text here..}

\end{comment}





\subsection{Stochastic adversaries}
\label{sec:ub-stoch}
In this section, we consider stochastic adversaries and present a reduction from private online learning problems---including OPE and online convex optimization (OCO) in general---to the (offline) differentially private stochastic convex optimization (DP-SCO)~\citep{BassilyFeTaTh19}. This reduction demonstrates that the (offline) DP-OCO problem is not harder than private online learning for stochastic adversaries: any algorithm for DP-SCO can be transformed into an online algorithm with stochastic adversaries with nearly the same rate (up to logarithmic factors). Using existing algorithms for DP-SCO~\citep{AsiFeKoTa21}, this reduction then results in regret $\sqrt{T\log d} +  \diffp^{-1} \log d \log T$ for private prediction from experts (\cref{cor:DP-exp-stoch}) and regret $\sqrt{T} + \diffp^{-1} \sqrt{d} \log T$ for general DP online convex optimization in $\ell_2$-geometry (\cref{cor:DP-OCO}).

Our reduction builds on algorithms for DP-SCO. In this problem, the loss functions are sampled i.i.d. from some distribution $\ell_i \simiid P$ where $\ell_i : \mc{X} \to \R$ and the goal is to minimize the population loss $L(x) = \E_{\ell \sim P}[\ell(x)]$ given $n$ samples $\ell_1,\dots,\ell_n \simiid P$. The performance of an algorithm $\A$ given $n$ samples is measured by its excess population loss, that is, $\Delta_n(\A) = \E[{L(\A(\ell_1,\dots,\ell_n)) - \inf_{x \in \mc{X}}L(x)}]$.

%In this section, we consider stochastic adversaries and study the more general DP-OCO problem (which includes prediction from experts). We show a reduction from DP-OCO to the offline DP-SCO problem which demonstrates that DP-OCO is not harder than DP-SCO for stochastic adversaries: any algorithm for DP-SCO can be transformed into an online algorithm for DP-OCO with stochastic adversaries with nearly the same rate (up to logarithmic factors). Using existing algorithms for DP-SCO~\cite{FeldmanKoTa20,AsiFeKoTa21}, this reduction then results in regret $\sqrt{T\log d} +  \frac{\log d \log T}{\diffp} $ for private prediction from experts (\cref{cor:DP-exp-stoch}) and regret $\sqrt{T} + \frac{\sqrt{d} \log T}{\diffp}$ for DP-OCO in $\ell_2$-geometry (\cref{cor:DP-OCO}).

%we show that stochastic adversaries results only in additional logarithmic penalty compared to the offline setting, that is, $O(\log(d) (\frac{1}{\sqrt{T}} + \log(T)/T\diffp))$ normalized regret. 
%Our upper bounds are based on a general reduction for DP-OCO with stochastic adversaries to DP-SCO that results in nearly the same utility guarantees (up to logarithmic factors).
Given an algorithm $\A$ for DP-SCO,
we design an online algorithm that updates the model only a logarithmic number of times---during the time-steps $t=1,2,4,8,\dots,T$.  For each such time-step $t$, we run $\A$ on the past $t/2$ samples to release the next model. As the loss functions are from the same distribution, the previous model generated by $\A$ should perform well for future loss functions. 
We present the full details in~\cref{alg:stoch-adv}.


\begin{algorithm}
	\caption{Limited Updates for Online Optimization with Stochastic Adversaries}
	\label{alg:stoch-adv}
	\begin{algorithmic}[1]
	    \REQUIRE Parameter space $\mc{X}$, DP-SCO algorithm $\A$
		\STATE Set $x_0 \in \mc{X}$ 
		
        \FOR{$t=1$ to $T$\,}
            \IF{$t=2^\ell$ for some integer $\ell \ge 1$}
                \STATE Run an optimal \ed-DP-SCO algorithm $\A$ over $\mc{X}$ with samples $\ell_{t/2},\dots,\ell_{t-1}$.
                % \begin{equation*}
                %     L_t(x) = \sum_{i=t/2}^{t-1} \ell_i(x)
                % \end{equation*}
                
                \STATE Let $x_t$ denote the output of the private algorithm
            \ELSE
                \STATE Let $x_t = x_{t-1}$
            \ENDIF
            \STATE Receive $\ell_t: \mc{X} \to \R$.
            \STATE Pay cost $\ell_t(x_t)$
            %\STATE $t = t + 1$
        \ENDFOR
	\end{algorithmic}
\end{algorithm}
We have the following regret for~\cref{alg:stoch-adv}. We defer the proof to~\cref{sec:thm-ub-stoch-OCO}.
\begin{theorem}
\label{thm:ub-stoch-OCO}
    Let $\ell_1,\dots,\ell_T : \mc{X} \to \R$ be convex functions chosen by a stochastic adversary, $\ell_i \simiid P$. 
    Let $\A$ be a \ed-DP algorithm for DP-SCO. Then
    \cref{alg:stoch-adv} is \ed-DP and has regret
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in \mc{X}} \sum_{t=1}^T \ell_t(x) \right]
        \le \sum_{i=1}^{\log T} 2^i \Delta_{2^i}(\A).
    \end{equation*}
\end{theorem}
% \begin{proof}
%     The privacy claim is immediate as each sample $\ell_i$ is used only once in running a single \ed-DP algorithm. Now we prove the claim about utility. Consider time-step $t=2^i$ where we invoke a DP-SCO algorithm with $t/2 = 2^{i-1}$ samples. 
%     Therefore the guarantees of the algorithm imply that at iteration $t$ we have
%     \begin{equation*}
%         \E_{\ell_t \sim P} \left[\ell_t(x_t) - \min_{x \in [d]} \ell_t(x) \right] \le O \left( \Delta_{2^i} \right).
%     \end{equation*}
%     Therefore at phase $i$, that is $2^{i} \le t \le 2^{i+1}$, the total regret is at most 
%     \begin{equation*}
%     \E\left[ \sum_{t=2^{i}}^{2^{i+1}}\ell_t(x_t) - \min_{x \in [d]} \sum_{t=2^{i}}^{2^{i+1}} \ell_t(x) \right] 
%         \le O \left(2^i \Delta_{2^i} \right).
%     \end{equation*}
%     Summing over $i$ proves the claim.
% \end{proof}

\newcommand{\Aopt}{\A_{\mathsf{\ell_2}}}
\newcommand{\Aone}{\A_{\mathsf{\ell_1}}}
Now we present the implications of this reduction for DP-OPE with stochastic adversaries. We use 
the algorithm for DP-SCO in $\ell_1$-geometry from~\cite{AsiFeKoTa21}. This algorithm, denoted $\Aone$, has excess population loss $\Delta_n(\Aone) = O(\sqrt{\log(d)/n} + \log(d)/n\diffp)$. We have the following result which we prove in~\cref{sec:apdx-cor-DP-exp-stoch}.
\begin{corollary}
\label{cor:DP-exp-stoch}
    Let $\ell_1,\dots,\ell_T : [d] \to [0,1]$ be  chosen by a stochastic adversary, $\ell_i \simiid P$. 
    %Let $\A$ be an optimal \ed-DP algorithm for DP-SCO with excess loss $O(\Delta_n)$ using $n$ samples. 
    Then
    \cref{alg:stoch-adv} using $\Aone$ is $\diffp$-DP and has regret
    \begin{equation*}
     \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
        \le  O \left(\sqrt{T\log d} +  \frac{\log d \log T}{\diffp} \right).
    \end{equation*}   
\end{corollary}

% We also have the following result DP-OCO in $\ell_2$-geometry. We use an optimal \ed-DP-SCO algorithm from~\cite{FeldmanKoTa20}, which we call $\Aopt$. As this algorithm has excess loss $\Delta_n = LD \cdot O(1/\sqrt{n} + \sqrt{d}/n\diffp)$, we obtain the following corollary. We defer the proof to~\cref{sec:apdx-cor-DP-OCO}. 
% \begin{corollary}(DP-OCO in $\ell_2$-geometry)
% \label{cor:DP-OCO}
%     Let $\mc{X} = \{ x \in \R^d: \ltwo{x} \le D\}$
%     and $\ell_1,\dots,\ell_T : \mc{X} \to \R$ be convex and $L$-Lipschitz functions chosen by a stochastic adversary, $\ell_i \simiid P$.
%     %Let $\A$ be an optimal \ed-DP algorithm for DP-SCO with excess loss $O(\Delta_n)$ using $n$ samples. 
%     Then
%     \cref{alg:stoch-adv} using $\Aopt$ is \ed-DP and has regret
%     \begin{equation*}
%      \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
%         \le LD \cdot O \left(\sqrt{T} + \frac{\sqrt{d} \log(T)}{\diffp} \right)
%     \end{equation*}   
% \end{corollary}



















% \subsection{Adaptive adversaries}
% \label{sec:adap-adv}
% For completeness, in this section we recall the known regret bounds for adaptive adversaries. \cite[section 5.2]{JainTh14} and~\cite{AgarwalSi17} (modified for approximate DP) give the following regret bounds.



% %In this section, we study adaptive adversaries and show algoriths with regret $O(\sqrt{T}/\diffp)$. This regret has been achieved by previous work using the exponential mechanism~\cite{}. Here we give a simple algorithm which is an instance of follow-the-perturbed-leader (FPL).



% %This was done in earlier work. here we have a simple algorithm based on follow the perturbed leader:
% % \begin{equation*}
% %     x_t = \argmin_{x \in [d]} \sum_{i=1}^{t-1} \ell_i(x) + \mathsf{Laplace}(\sqrt{T}/\diffp).
% % \end{equation*}


% %The utility guarantees of FPL immediately give the following theorem.
% \begin{theorem}\cite{JainTh14,AgarwalSi17}
% \label{thm:ub-adap}
%     Let $\ell_1,\dots,\ell_T \in [0,1]^d$ be chosen by an adaptive adversary. %\cref{alg:adap-adv} with $\Delta = \sqrt{T}/\diffp$ is \ed-DP and has regret
%     There is an \ed-DP algorithm that has regret \hac{verify log factors in the $\sqrt{d}$ term}
%     \begin{equation*}
%      \E\left[ \sum_{t=1}^T \ell_t(x_t) - \min_{x \in [d]} \sum_{t=1}^T \ell_t(x) \right]
%         \le O \left(\sqrt{T\log(d)} +  \min \left( \frac{\sqrt{T \log(1/\delta) \log(d)}}{\diffp}  , \frac{\sqrt{d \log(1/\delta)} \log (d) \log^2(T)}{\diffp} \right) \right).
%     \end{equation*}
% \end{theorem}
% \begin{proof}
%     The utility analysis follows immediately from the utility guarantees of FPL~\cite[theorem ?]{KalaiVe05} \hac{good reference for this with adaptive adversaries?}. The privacy guarantee follows from advanced composition as report-noisy-max implies that each iterate is $\diffp/\sqrt{T}$-DP.
% \end{proof}


% \begin{algorithm}
% 	\caption{Private FPL}
% 	\label{alg:adap-adv}
% 	\begin{algorithmic}[1]
% 	    \REQUIRE Noise parameter $\Delta > 0$
% 		\STATE Set $x_0 = 1$
%         \FOR{$t=1$ to $T$\,}
%             \STATE Sample $p_t \sim \lap(\Delta)^d$
%             %$p_0(x_t) + \sum_{i=1}^{t-1} \ell_i(x_t) < p_0(x) + \sum_{i=1}^{t-1} \ell_i(x) - 2/\diffp$ for all other $x \in [d]$
%             %\IF{Sparse-Vec identifies above thershold}
%             \STATE $x_t = \argmin_{x \in [d]} p_t(x) + \sum_{i=1}^{t-1} \ell_i(x) $
%             %\ENDIF
%             \STATE Receive $\ell_t \in \R^d$
%             \STATE Pay cost $\ell_t(x_t)$
%         \ENDFOR
% 	\end{algorithmic}
% \end{algorithm}
